Query and Extract: Refining Event Extraction as Type-oriented Binary Decoding

Event extraction is typically modeled as a multi-class classification problem where event types and argument roles are treated as atomic symbols. These approaches are usually limited to a set of pre-defined types. We propose a novel event extraction framework that uses event types and argument roles as natural language queries to extract candidate triggers and arguments from the input text. With the rich semantics in the queries, our framework benefits from the attention mechanisms to better capture the semantic correlation between the event types or argument roles and the input text. Furthermore, the query-and-extract formulation allows our approach to leverage all available event annotations from various ontologies as a unified model. Experiments on ACE and ERE demonstrate that our approach achieves state-of-the-art performance on each dataset and significantly outperforms existing methods on zero-shot event extraction.

==> ACL 2022_ Refining Event Extraction as Type-oriented Binary Decoding/1intro.tex <==
\section{Introduction}
\label{sec:intro}


Event extraction~\cite{grishman1997information,chinchor1998muc,ahn2006stages} is a task to identify and type event triggers and participants from natural language text. As shown in
Figure~\ref{fig:intro_example}, \textit{married} and \textit{left} are triggers of two event mentions of the \textit{Marry} and \textit{Transport} event types respectively. Two arguments are involved in the \textit{left} event mention: \textit{she} is an \textit{Artifact}, and \textit{Irap} is the \textit{Destination}.



Traditional studies usually model event extraction as a multi-class classification 
problem~\cite{mcclosky2011event,qiliACl2013,chen2015event,yang-mitchell-2016-joint,nguyen_jrnn_2016,yinglinACL2020}, where a set of event types are first defined, and then supervised machine learning approaches will detect and classify each candidate event mention or argument into one of the target types. However, each event type or argument role is treated as an atomic symbol, ignoring their rich semantics in these approaches. Several studies explore the semantics of event types by leveraging the event type structures~\cite{huang2017zero}, seed event mentions~\cite{bronstein2015seed,lai2019extending}, or question answering (QA)~\cite{xinyaduEMNLP2020,jianliu2020emnlp}.
However, these approaches are still designed for and thus limited to a single target event ontology\footnote{An ontology is defined as a collection of event types and argument roles for a particular domain \cite{brown-etal-2017-rich, song2015light}.}, such as ACE~\cite{ldc_ace05} or ERE~\cite{song2015light}.


\begin{figure}
% \vspace{8mm}
  \centering
  \includegraphics[width=0.45\textwidth]{example-1.png}
  \caption{An example of event annotation.}
  \label{fig:intro_example}
\end{figure}

With the existence of multiple ontologies and the challenge of handling new emerging event types, it is necessary to study event extraction approaches that are generalizable and can use all available training data from distinct event ontologies.\footnote{For argument extraction, the QA-based approaches have certain potential to generalize to new ontologies, but require high-quality template questions. As shown in our experiments, their generalizability is limited compared to ours.}


\begin{figure*}
  \centering
  \includegraphics[width=0.91\textwidth]{EEQA_architecture.png}
  \caption{Architecture overview. Each cell in Argument Role Score Matrix indicates the probabilities of an entity being labeled with an argument role. The arrows in Multiway Attention module show four attention mechanisms: (a) entity to argument roles, (b) argument role to entities, (c) entity to entities, (d) argument role to argument roles.}
  \label{fig:architecture}
\end{figure*}

To this end,
we propose a new event extraction framework following a query-and-extract paradigm.
Our framework represents event types and argument roles as natural language queries with rich semantics.
The queries are then used to extract the corresponding event triggers and arguments by leveraging our proposed attention mechanism to capture their interactions with input texts. Specifically, (1) for trigger detection, we formulate each event type as a query based on its type name and a short list of prototype triggers, and make \textbf{binary decoding} of each token based on its query-aware embedding; (2) for argument extraction, we put together all argument roles defined under each event type as a query, followed by a multiway attention mechanism to extract all arguments of each event mention with \textbf{one-time encoding}, with each argument predicted as \textbf{binary decoding}.



Our approach can naturally handle various ontologies as a unified model --
compared to previous studies~\cite{nguyen-grishman-2016-modeling,wadden-etal-2019-entity,yinglinACL2020}, our binary decoding mechanism directly works with any event type or argument role represented as natural language queries, thus effectively leveraging cross-ontology event annotations and making zero-shot predictions.
Moreover, compared with the QA-based methods~\cite{xinyaduEMNLP2020,jianliu2020emnlp,EEMQA_li} that can also conduct zero-shot argument extraction, our approach does not require creating high-quality questions for argument roles or multi-time encoding for different argument roles separately, thus being more accurate and efficient.

We evaluate our approach on two public benchmark datasets, ACE and ERE, and demonstrate state-of-the-art performance in the standard supervised event extraction and the challenging transfer learning settings that generalize to new event types and ontologies. Notablely, on zero-shot transfer to new event types, our approach outperforms a strong baseline by 16\% on trigger detection and 26\% on argument detection. The overall contributions of our work are:

\begin{itemize}%[noitemsep,nolistsep,wide,itemindent=3pt]
 
\item We refine event extraction as a query-and-extract paradigm, which is more generalizable and efficient than previous top-down classification or QA-based approaches. 

\item We design a new event extraction model that leverages rich semantics of event types and argument roles, improving accuracy and generalizability. 

\item We establish new state-of-the-art performance on ACE and ERE in supervised and zero-shot event extraction and demonstrate our framework as an effective unified model for cross ontology transfer.
% and demonstrate our framework as a more efficient and accurate unified model that can make use of event annotations from different ontologies and extract events for any unseen types.
\end{itemize}


==> ACL 2022_ Refining Event Extraction as Type-oriented Binary Decoding/2model.tex <==
\section{Our Approach}
\label{sec:model}

%\lifu{add a figure to show the overall approach}
%\lifu{briefly describe the overview of the approach}

As Figure~\ref{fig:architecture} shows, given an input sentence, we first identify the candidate triggers for each event type by taking it as a query to the sentence. Each event type, such as \textit{Attack}, is represented with a natural language text, including its type name and a shortlist of prototype triggers, such as \textit{invaded} and \textit{airstrikes}, %\textit{overthrew}, and \textit{ambushed}, 
which are selected from the training examples. Then, we concatenate the input sentence with the event type query, encode them with a pre-trained BERT encoder~\cite{devlin-etal-2019-bert}, compute the attention distribution over the sequential representation of the event type query for each input token, and finally classify each token into a binary label, indicating it as a trigger candidate of the specific event type or not. 

To extract the arguments for each candidate trigger, we follow a similar strategy and take the set of pre-defined argument roles for its corresponding event type as a query to the input sentence. We use another BERT encoder to learn the contextual representations for the input sentence and the query of the argument roles. Then, we take each entity of the input sentence as a candidate argument and compute the semantic correlation between entities and argument roles with multiway attention, and finally classify each entity into a binary label in terms of each argument role. 

% As Figure~\ref{fig:architecture} shows, given an input sentence $W = \{w_{1}, w_{2}, \dots, w_{n} \}$, we first identify the candidate event triggers for each event type $t \in \mathcal{T}$ where $\mathcal{T}$ denotes the target event ontology. Each event type $t$, such as \type{Attack}, is also associated with a list of seed triggers, such as \textit{invaded}, \textit{airstrikes}, which are selected from the annotated training data. To detect candidate triggers for each event type $t$, we use a pre-trained BERT~\cite{devlin-etal-2019-bert} to encode the input sentence, the event type as well as its seed triggers, compute enriched attention, and classify each input token into a binary label. 

% Given an event trigger of type $t$, to extract arguments, we concatenate the input sentence $W$ with all argument roles $Arg^t = \{arg^t_1, arg^t_2, ..., arg^t_d\}$ for event type $t$, and encode them with another pre-trained BERT model. Then, we identify the entities  ${E} = \{{en}_1, {en}_2, \dots, {en}_k\}$ from the input sentence and classify each entity into a particular argument role with a XXX.

%. Entities that have a strong correlation with the event trigger are taggable event arguments. Then we calculate enriched attention and classify entities into argument roles using table decoding.

%we take the concatenation of the given sentence $W$ and argument roles  $Arg^t = \{arg^t_1, arg^t_2, ..., arg^t_d\}$ for the event $t$ as input to the argument detection model and encode it by a pre-trained BERT. We identify the entities  ${E} = \{{en}_1, {en}_2, \dots, {en}_k\}$ in the given sentence. Entities that have a strong correlation with the event trigger are taggable event arguments. Then we calculate enriched attention and classify entities into argument roles using table decoding. 

% At inference time, ...

% overall architecture
% \begin{figure*}
%   \centering
%   \includegraphics[width=\textwidth]{3Model/EEQA architecture3.png}
% %   \makebox[\textwidth][c]{\includegraphics[width=1.2\textwidth]{3Model/EEQA architecture.png}}
%   \caption{The overall architecture of our proposed approach. Argument role score matrix stores scores for each entity being labeled as the target argument role. The arrows in multiway attention module indicates four attention directions: (a) entity to argument roles, (b) argument tole to entities, (c) entity to the rest entities and (d) argument role to the rest argument roles.}
%   \label{fig:architecture}
% \end{figure*}

\subsection{Trigger Detection}

%\lifu{use mathematical language to describe the process. Check previous papers, e.g., the OneIE paper}

% \lifu{you can divide the approach into several components, e.g., event type representation to describe how to get the anchor words and represent each type, context encoding, attention, event trigger prediction, etc. Add detailed formulas for each step}

\paragraph{Event Type Representation} A simple and intuitive way of representing an event type is to use the type name. However, the type name itself cannot accurately represent the semantics of the event type due to the ambiguity of the type name and the variety of the event mentions of each type. For example, \textit{Meet} can refer to \textit{an organized event} or an action of \textit{getting together} or \textit{matching}. Inspired by previous studies~\cite{bronstein2015seed,lai2019extending}, we use a short list of prototype triggers to enrich the semantics of each event type.
%, and more than 60 unique strings are annotated as \textit{Meet} event triggers in ACE05 dataset

%Previous studies either treat each event type as an atomic symbol~\cite{} or represent it with the type name only~\cite{jianliu2020emnlp, yinglinACL2020, xinyaduEMNLP2020}. Few studies explored seed triggers to denote the semantics of each event type and applied them to few-shot event extraction~\cite{}. Following similar intuitions, for each event type, we carefully select $K$ seed triggers from the training examples and use them to enrich the semantics of each event type.

%~\cite{jianliu2020emnlp, yinglinACL2020, xinyaduEMNLP2020} mainly rely on the type name to denote the semantics of each event type. 
%However, it's impossible for an event type name, which usually consists of two to three words, to cover the event type semantics. On the other hand, supplementary knowledge of each event type can be retrieved from the training data. For each event type, a collection of words or phrases are frequently labeled as triggers. Those words and phrases, named as seed triggers, are representative of the event type. 

%Thus we further select $K$ seed triggers $tr_1^{seed}\; tr_2^{seed}\; \dots tr_K^{seed} $  from the training examples based on two factors, term frequency and positive rate (in being tagged as an event trigger).

Specifically, for each event type $t$, we collect a set of annotated triggers from the training examples. For each unique trigger word, we compute its frequency from the whole training dataset as $f_o$ and its frequency of being tagged as an event trigger of type $t$ as $f_t$, and then obtain a probability $f_t/f_o$, which will be used to sort all the annotated triggers for event type $t$. We select the top-$K$\footnote{In our experiments, we set $K=4$.} ranked words as prototype triggers $\{\tau_1, \tau_2, \dots, \tau_K\}$. 

Finally, each event type will be represented with a natural language sequence of words, consisting of its type name and the list of prototype triggers $T= \{t, \tau_1^t, \tau_2^t, \dots, \tau_K^t\}$. Taking the event type \textit{Attack} as an example, we finally represent it as \textit{Attack invaded airstrikes overthrew ambushed}.

%each trigger mention, and its positive rate in being tagged as event trigger. We filter out less frequent trigger mentions, and select up to $K$ seed triggers with highest positive rate. \lifu{provide details: which numbers you computed, and how to rank them...}\sijia{ added}

%we sort the event trigger mentions from the training data by positive rates, and take the most frequent ones as seed triggers. For example, we choose \textit{invaded}, \textit{airstrikes}, \textit{overthrew}, and \textit{ambushed} as seed triggers for event type \textsc{attack}.

% \paragraph{Event Question Strategy.}
\paragraph{Context Encoding}
% \lifu{are you using POS tags? confirm}\sijia{I concatenate them before the last MLP layer}
Given an input sentence $W = \{w_{1}, w_{2}, \dots, w_{N} \}$, we take each event type $T= \{t, \tau_1^t, \tau_2^t, \dots, \tau_K^t\}$ as a query to extract the corresponding event triggers. Specifically, we first concatenate them into a sequence as follows:
\begin{gather*}
\text{[CLS]} \text{[EVENT]} \text{[SEP]}\; w_{1}\; ...\; w_{N}\; \text{[SEP]}\; \\t\; \tau_1^t\; ...\; \tau_K^t\;  \text{[SEP]}
\end{gather*}
% For each event type, we ask whether an token indicate such event by a question with the following three parts: 
where [SEP] is a separator from the BERT encoder~\cite{devlin-etal-2019-bert}. Following ~\cite{jianliu2020emnlp}, we use a special symbol [EVENT] to emphasis the trigger detection task. %as part of event type queries

Then we use a pre-trained BERT encoder to encode the whole sequence and get contextual representations for the input sentence $\boldsymbol{W} = \{\boldsymbol{w}_0, \boldsymbol{w}_2, ..., \boldsymbol{w}_N\}$ as well as the event type $ \boldsymbol{T} = \{\boldsymbol{t}, \boldsymbol{\tau}_0^t, \boldsymbol{\tau}_1^t, ..., \boldsymbol{\tau}_K^t\}$.\footnote{We use bold symbols to denote vectors.}

%The sequence connects the following three components  with special token [CLS] and [SEP] \cite{devlin-etal-2019-bert}:
%(i) a special token $\text{[EVENT]}$ to emphasis the trigger detection task. (ii) the context sequence $w_{1}\; w_{2}\; \dots w_{N}$. (iii) an event type query with event type name $ev_1 \;  ev_2$ and seed triggers $tr_1^{seed}\; tr_2^{seed}\; \dots tr_K^{seed} $. 
%For instance, as the example in Figure \ref{fig:architecture}, in the input sequence 
%"{[CLS] [EVENT] [SEP] The convoy was escorted by U.S. soldiers [SEP] transport arrival travels expelled [SEP]}", "transport" is the event sub-type token, and  "arrival travels expelled" are seed triggers. 
% \begin{displayquote}
% {[CLS] [EVENT] [SEP] Sentence [SEP] Event\_type Anchor\_words [SEP]}.
% \end{displayquote}
% where \textsc{[sep]} is the separator connecting the four parts, and \textsc{[cls]} is the special token indicate the start of the context. 



% \paragraph{Enriched Trigger Attention}
\paragraph{Enriched Contextual Representation}
%Different from previous studies~\cite{}, we aim to take each event type as query to an input sentence and detect candidate triggers by capturing the correlation between each token and the event type. 
Given a query of each event type, we aim to automatically extract corresponding event triggers from the input sentence. To achieve this goal, we need to capture the semantic correlation of each input token to the event type. Thus we apply attention mechanism to learn a weight distribution over the sequence of contextual representations of the event type query and get an event type aware contextual representation for each token:
%compute the relevance of each input token to the event type and learn an event type oriented contextual representation for each token.
%After obtaining the contextual representations, we aim to detect event triggers for each event type. To do so, we first learn an event type oriented contextual representation for each token based on the following attention mechanism:
% \begin{small}
\begin{gather*}
    \boldsymbol{A}_{i}^{T} = \frac{1}{T}\sum_{j=1}^{|T|}\alpha_{ij}\cdot\boldsymbol{T}_j \;,\\\alpha_{ij} = \cos(\boldsymbol{w}_i,\ \boldsymbol{T}_j)\;,
% \belowdisplayskip=1pt
\end{gather*}
% \end{small}
where $\boldsymbol{T}_j$ is the contextual representation of the $j$-th token in the sequence $T= \{t, \tau_1^t, \tau_2^t, \dots, \tau_K^t\}$. $\cos(\cdot)$ is the cosine similarity function between two vectors. $\boldsymbol{A}_{i}^{T}$ denotes the event type $t$ aware contextual representation of token $w_i$.

In addition, the prediction of event triggers also depends on the occurrence of a particular context. For example, according to ACE event annotation guidelines~\cite{ldc_ace05}, to qualify as a \textit{Meet} event, the meeting must be known to be ``\textit{face-to-face and physically located somewhere}''. To capture such context information, we further apply in-context attention to capture the meaningful contextual words for each input token: 
%Taking \textit{Meet} event type as an example, some event types also require the occurrence of certain entities or context, for example, according to ACE2005 annotation guideline, to qualify as a \textit{Meet} Event, the meeting must be known to be face-to-face and physically located somewhere. To capture such context information, we further employ another in-context attention to capture meaningful contextual words for event type prediction: 
\begin{gather*}
    \boldsymbol{A}_{i}^W = \frac{1}{N}\sum_{j=1}^{N} \tilde{\alpha}_{ij}\cdot\boldsymbol{w}_j \; ,\\ \tilde{\alpha}_{ij} = \rho(\boldsymbol{w}_i,\ \boldsymbol{w}_j)\;,
\end{gather*}
where $\rho(.)$ is the attention function and is computed as the average of the self-attention weights from the last $m$ layers of BERT.\footnote{We set $m$ as 3 as it achieved the best performance.}


\paragraph{Event Trigger Detection}

With the event type oriented attention and in-context attention mechanisms, each token $w_i$ from the input sentence will obtain two enriched contextual representations $\boldsymbol{A}_{i}^W$ and $\boldsymbol{A}_{i}^{T}$. We concatenate them with the original contextual representation $\boldsymbol{w}_i$ from the BERT encoder, and classify it into a binary label, indicating it as a candidate trigger of event type $t$ or not:%\lifu{if you use pos tag features here, add it.}\sijia{added}
\begin{align*}
\small
   \boldsymbol{\tilde{y}}_i^t = \boldsymbol{U}_{o}\cdot([\boldsymbol{w}_i;\ \boldsymbol{A}_{i}^W;\ \boldsymbol{A}_{i}^{T}; \boldsymbol{P}_i]) \;,
\end{align*}
where $[;]$ denotes concatenation operation, $\boldsymbol{U}_{o}$ is a learnable parameter matrix for event trigger detection, and $\boldsymbol{P}_i$ is the one-hot part-of-speech (POS) encoding of word $w_i$. We optimize the following objective for event trigger detection
\begin{align*}
\small
    % L & = -\frac{1}{|\mathcal{T}|}\sum_{t\in\mathcal{T}}L^t_{trigge}\\
    \mathcal{L}_{1} = -\frac{1}{|\mathcal{T}||\mathcal{N}|}
        \sum_{t\in\mathcal{T}}
        \sum_{i=1}^{|\mathcal{N}|} \boldsymbol{y}_i^t\cdot\log \boldsymbol{\tilde{y}}_i^t\;,
\end{align*}
where $\mathcal{T}$ is the set of target event types and $\mathcal{N}$ is the set of tokens from the training dataset. $\boldsymbol{y}_i^t$ denotes the groundtruth label vector.

\subsection{Event Argument Extraction}
After detecting event triggers for each event type, we further extract their arguments based on the pre-defined argument roles of each event type.

\paragraph{Context Encoding}
Given a candidate trigger $r$ from the sentence $W = \{w_{1}, w_{2}, \dots, w_{N} \}$ and its event type $t$, we first obtain the set of pre-defined argument roles for event type $t$ as $G^t = \{g^t_1, g^t_2, ..., g^t_D\}$. To extract the corresponding arguments for $r$, similar as event trigger detection, we take all argument roles $G^t$ as a query and concatenate them with the original input sentence
\begin{align*}
    \text{[CLS]}\; w_{1}\; w_{2}\; ...\; w_{N}\; \text{[SEP]}\; g^t_1\; g^t_2\; ...\; g^t_D\; \text{[SEP]}
\end{align*}
where we use the last \text{[SEP]} separator to denote \textit{Other} category, indicating the entity is not an argument. 
Then, we encode the whole sequence with another pre-trained BERT encoder~\cite{devlin-etal-2019-bert} to get the contextual representations of the sentence $\boldsymbol{\tilde{W}} = \{\boldsymbol{\tilde{w}}_0, \boldsymbol{\tilde{w}}_2, ..., \boldsymbol{\tilde{w}}_N\}$, and the argument roles $ \boldsymbol{G}^t = \{\boldsymbol{g}_0^t, \boldsymbol{g}_1^t, ..., \boldsymbol{g}_D^t, \boldsymbol{g}_{\text{[Other]}}^t\}$.

As the candidate trigger $r$ may span multiple tokens within the sentence, we obtain its contextual representation $\boldsymbol{r}$ as the average of the contextual representations of all tokens within $r$. In addition, as the arguments are usually detected from the entities of sentence $W$, we apply a BERT-CRF model, which is optimized on the same training set as event extraction to identify the entities $E=\{e_1, e_2, ..., e_M\}$. As each entity may also span multiple tokens, following the same strategy, we average the contextual representations of all tokens within each entity and obtain the entity contextual representations as $\boldsymbol{E}=\{\boldsymbol{e}_1, \boldsymbol{e}_2, ..., \boldsymbol{e}_M\}$.


\paragraph{Multiway Attention} 

Given a candidate trigger $r$ of type $t$ and an entity $e_i$, for each argument role $g^t_{j}$, we need to determine whether the underlying relation between $r$ and $e_i$ corresponds to $g^t_{j}$ or not, namely, whether $e_i$ plays the argument role of $g^t_{j}$ in event mention $r$. To do this, for each $e_i$, we first obtain a trigger-aware entity representation as 
\begin{align*}
    \boldsymbol{h}_{i} = \boldsymbol{U}_{h}\cdot([\boldsymbol{e}_{i};\ \boldsymbol{r};\ \boldsymbol{e}_{i}\circ\boldsymbol{r}]) \;,
\end{align*}
where $\circ$ denotes element-wise multiplication operation. $\boldsymbol{U}_{h}$ is a learnable parameter matrix.

In order to determine the semantic correlation between each argument role and each entity, we first compute a similarity matrix $\boldsymbol{S}$ between the trigger-aware entity representations $\{\boldsymbol{h}_1, \boldsymbol{h}_2, ..., \boldsymbol{h}_M\}$ and the argument role representations $\{\boldsymbol{g}_0^t, \boldsymbol{g}_1^t, ..., \boldsymbol{g}_D^t\}$
\begin{align*}
    S_{ij} = \frac{1}{\sqrt{d}}\sigma(\boldsymbol{h}_{i},\   \boldsymbol{g}^{t}_{j})\;,
\end{align*}
where $\sigma$ denotes dot product operator, $d$ denotes embedding dimension of $\boldsymbol{g}^t$, and $S_{ij}$ indicates the semantic correlation of entity $e_i$ to a particular argument role $g^t_{j}$ given the candidate trigger $r$.

Based on the correlation matrix $\boldsymbol{S}$, we further apply a bidirectional attention mechanism to get an argument role aware contextual representation for each entity and an entity-aware contextual representation for each argument role as follows:  
\begin{gather*}
    \boldsymbol{A}^{e2g}_{i} = \sum_{j=1}^{D} \boldsymbol{S}_{ij}\cdot\boldsymbol{g}_{j}^{t}\;, \\
    \boldsymbol{A}^{g2e}_{j} = \sum_{i=1}^{M} \boldsymbol{S}_{ij}\cdot\boldsymbol{h}_{i}\;.
\end{gather*}

In addition, previous studies~\cite{hong2011using,qiliACl2013,yinglinACL2020} have revealed that the underlying relations among entities or argument roles are also important to extract the arguments. For example, if entity $e_1$ is predicted as \textit{Attacker} of an \textit{Attack} event and $e_1$ is \textit{located in} another entity $e_2$, it's very likely that $e_2$ plays an argument role of \textit{Place} for the \textit{Attack} event. To capture the underlying relations among the entities, we further compute the self-attention among them
\begin{align*}
    \mu_{ij} =\frac{1}{\sqrt d}\sigma(&\boldsymbol{h}_{i},\ \boldsymbol{h}_{j})  \;, \,\,\,\,\,\, \boldsymbol{\tilde{\mu}}_{i} = \text{Softmax}(\boldsymbol{\mu}_{i})\;, \\
    % & \boldsymbol{\tilde{\mu}}_{i} = \text{Softmax}(\boldsymbol{\mu}_{i})\;, \\
    &\boldsymbol{A}^{e2e}_{i} = \sum_{j=1}^{M}
    \tilde{\mu}_{ij}\cdot\boldsymbol{h}_{j}\;. 
    %  \boldsymbol{A}^{e2e}_{k} = &\frac{1}{|I_{e_k}|} \sum\nolimits_{j\in I_{e_k}}\sum\nolimits_i
    % {\mu}_{ij}\cdot\boldsymbol{h}_{i}\;,
    % \\
    % & \boldsymbol{A}^{e2e}_{i} = \boldsymbol{h}_{j}^{\top}\cdot\text{Softmax}(\boldsymbol{\mu}_{i})\;,
\end{align*}

Similarly, to capture the underlying relations among argument roles, we also compute the self-attention among them
\begin{align*}
    v_{jk} = \frac{1}{\sqrt{d}}\sigma(\boldsymbol{g}^{t}_{j} & ,\  \boldsymbol{g}^{t}_{k})\;,  \,\,\,\,\,\,
    \boldsymbol{\tilde{v}}_{j} = \text{Softmax}(\boldsymbol{v}_{j})\;, \\
    & \boldsymbol{A}^{g2g}_{j} = \sum_{k=1}^{D}
    \tilde{v}_{jk}\cdot\boldsymbol{g}_{k}^{t}\;.
\end{align*}

\paragraph{Event Argument Predication} Finally, for each candidate event trigger $r$, we determine whether an entity $e_i$ plays an argument role of $g^{t}_{j}$ in the event mention by classifying it into a binary class:
\begin{align*}
    \boldsymbol{\tilde{z}}^{t}_{ij} = \boldsymbol{U}_{a}\cdot([\boldsymbol{h}_{i};\ \boldsymbol{g}^{t}_{j};\ \boldsymbol{A}^{e2g}_{i};\ \boldsymbol{A}^{g2e}_{j};\ \boldsymbol{A}^{e2e}_{i};\ \boldsymbol{A}^{g2g}_{j}]) ,
\end{align*}
where $\boldsymbol{U}_{a}$ is a learnable parameter matrix for argument extraction. And $\tilde z^t$ is argument role score matrix for event type $t$. The training objective is to minimize the following loss function:
\begin{align*}
   \mathcal{L}_{2} = -\frac{1}{|\mathcal{A}||\mathcal{E}|}
        \sum_{j=1}^{|\mathcal{A}|}
        \sum_{i=1}^{|\mathcal{E}|} \boldsymbol{z}_{ij} \log \boldsymbol{\tilde{z}}_{ij}\;,
\end{align*} 
where $\mathcal{A}$ denotes the collection of possible argument roles, and $\mathcal{E}$ is the set of entities we need to consider for argument extraction. $\boldsymbol{z}_{ij}$ denotes the ground truth label vector. During test, an entity will be labeled as a non-argument if the prediction for \textit{Other} category is 1. Otherwise, it can be labeled with multiple argument roles.


==> ACL 2022_ Refining Event Extraction as Type-oriented Binary Decoding/3experiments.tex <==
\section{Experiments}
\label{sec:exp}

% \lifu{** Another possible comment from reviewers could be: QA based approaches can leverage QA annotations. However, it seems our approach cannot. Should we also try to incorporate QA datasets for pretraining?}

%We compare our approach with existing baselines in both standard supervised learning settings and transfer learning settings. 

% \begin{table}
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% Dataset &  Split & \# Events & \# Arguments
%  \\
% \midrule
% \multirow{3}{*}{ACE}
%     & Training &  4419  & 7932\\
%     & Development   &  468   & 892 \\
%     & Test  &  424   & 898 \\
% \midrule
% \multirow{3}{*}{ERE}
%     & Training & 7232  & 12832 \\
%     & Development   & 619   & 1100  \\
%     & Test  & 652   & 1228  \\
% \bottomrule
% \end{tabular}
% \caption{Data statistics for ACE2005 and ERE datasets.}
% \label{tab:data statistics}
% \end{table}


%ACE defines 7 entity types, 33 event types, 22 argument role (or 28 argument roles with time and value argument roles). And there are 7 entity types, 38 event types, 21 argument role (or 26 argument roles with time and value argument roles) in ERE-EN. Time related argument roles such as Time-Within and Time-Starts are collapsed into one Time role. For ACE-EN, we use the same data split as the previous work~\cite{qiliACl2013, DMCNN_chen2015, psl_liu2016, yang-mitchell-2016-joint, nguyen-grishman-2016-modeling, wadden-etal-2019-entity, jianliu2020emnlp, xinyaduEMNLP2020}. 
%This data split includes 529 documents for training set, 30 documents for development set and 40 articles for test set. For ERE-EN, we use the same data split as ~\cite{yinglinACL2020, vannguyen2021crosstask}, which includes 396 documents as training set, 31 documents as development set, and 31 document as test set. The details of the data statistics are in Table \ref{tab:data statistics}.


% \begin{table}
% \centering
% \small
% \begin{tabular}{lcrrr}
% \toprule
% Dataset &  Split & \# events & \# args & \# args (VT)*
%  \\
% \midrule
% \multirow{3}{*}{ACE}
%     & Train &  4419 &   6605    & 7932\\
%     & Dev   &  468  &   759     & 892 \\
%     & Test  &  424  &   689     & 898 \\
% \midrule
% \multirow{3}{*}{ERE}
%     & Train & 7232  &   11670   & 12832 \\
%     & Dev   & 619   &   983     & 1100  \\
%     & Test  & 652   &   1086    & 1228  \\
% \bottomrule
% \end{tabular}
% \caption{Data statistics for ACE2005 and ERE datasets. *args (VT) denotes arguments including values and times}
% \label{tab:data statistics}
% \end{table}



% \begin{table*}
% \centering
% \small
% \begin{tabular}{l|c|c|c|c|c|c}
% \toprule
% \multirow{2}{*}{Model}&  
% \multicolumn{2}{c|}{ACE05-E}&
% \multicolumn{2}{c|}{ACE05-E$^+$} &  
% \multicolumn{2}{c}{ERE}
% \\\cmidrule{2-7}&Tr. Ext. & Arg. Ext. & Tr. Ext. & Arg. Ext. & Tr. Ext. & Arg. Ext.
%  \\
% \midrule
%     %JointBeam \cite{qiliACl2013} & 67.5 & 41.8 & 52.7 & - \\
%     % JRNN \cite{nguyen_jrnn_2016} &69.3\\
%     % dbRNN~\cite{dbrnn_sha_2018} & 69.6 & 50.1 & 58.7 & - \\
%     DYGIE++~\cite{wadden-etal-2019-entity} & 69.7 & 48.8 &-&-& - & - \\
%     BERT\_QA\_Arg~\cite{xinyaduEMNLP2020}& 72.4 & 53.1 &70.6* & 48.3* & 57.0 & 39.2\\
%     OneIE~\cite{yinglinACL2020}&74.7 & 56.8 & 72.8 & 54.8 & 57.0  & 46.5 \\
%     Text2Event~\cite{text2event}&71.9&53.8 &71.8 & 54.4 & 59.4 & 48.3 \\
%     FourIE~\cite{vannguyen2021crosstask}&\textbf{75.4}&58.0 & 73.3 & \textbf{57.5} &  57.9  & 48.6 \\
%     % MQAEE ~\cite{EEMQA_li} &71.7 & 53.4 & - & - \\
%     %RCEE \cite{jianliu2020emnlp} & 74.9*? & 58.7? & ? & ? \\
% \midrule    
%     % \textbf{Query\&Extract} & \textbf{73.7} & 55.1 & \textbf{59.7} & \textbf{67.2}\\
%     % Our Approach w/o (Multiway) Attention&& & 72.2 & 54.0  & 55.6  & 42.2 \\
%     \textbf{Our Approach}&75.0 (?) &  & \textbf{73.7} & 55.1 &  \textbf{60.4}  & \textbf{50.2}\\
% \bottomrule
% \end{tabular}
% \caption{Event extraction results on ACE05 dataset and ERE dataset  (F-score, \%). % Argument Ext. (GE) indicates the argument extraction results with gold entities and system predicted triggers. Argument Ext. (GT) indicates the argument extraction performance with gold triggers and system detected entities. 
% % *indicate with data augmentation. 
% %$^{\star}$ indicates statistical significance $(p < 0.05)$.
% }
% \label{tab:ACE}
% \end{table*}


\begin{table*}
\centering
\small
\resizebox{0.8\textwidth}{!}
{
\begin{tabular}{l|c|c|c|c}
\toprule
\multirow{2}{*}{Model}&  
\multicolumn{2}{c|}{ACE05-E$^+$} &  
\multicolumn{2}{c}{ERE-EN}
\\
\cmidrule{2-5}
&Trigger Ext. & Argument Ext. & Trigger Ext. & Argument Ext. 
 \\
\midrule
    %JointBeam \cite{qiliACl2013} & 67.5 & 41.8 & 52.7 & - \\
    % JRNN \cite{nguyen_jrnn_2016} &69.3\\
    % dbRNN~\cite{dbrnn_sha_2018} & 69.6 & 50.1 & 58.7 & - \\
    DYGIE++~\cite{wadden-etal-2019-entity}  & 67.3$^*$ & 42.7$^*$ & - & - \\
    BERT\_QA\_Arg~\cite{xinyaduEMNLP2020}&70.6$^*$ & 48.3$^*$ & 57.0 & 39.2\\
    OneIE~\cite{yinglinACL2020} & 72.8 & 54.8 & 57.0  & 46.5 \\
    Text2Event~\cite{text2event} &71.8 & 54.4 & 59.4 & 48.3 \\
    FourIE~\cite{vannguyen2021crosstask}&73.3 & \textbf{57.5} &  57.9  & 48.6 \\
    % MQAEE ~\cite{EEMQA_li} &71.7 & 53.4 & - & - \\
    %RCEE \cite{jianliu2020emnlp} & 74.9*? & 58.7? & ? & ? \\
\midrule    
    % \textbf{Query\&Extract} & \textbf{73.7} & 55.1 & \textbf{59.7} & \textbf{67.2}\\
    % Our Approach w/o (Multiway) Attention&& & 72.2 & 54.0  & 55.6  & 42.2 \\
    % \textbf{Our Approach}& \textbf{73.7} & 55.1(55.6) &  \textbf{60.4}  & \textbf{50.2} (50.8)\\
        \textbf{Our Approach} & \textbf{73.6} (0.2) & 55.1 (0.5) &  \textbf{60.4} (0.3) & \textbf{50.4} (0.3)\\
\bottomrule
\end{tabular}
}
\caption{Event extraction results on ACE05-E$^+$ and ERE-EN datasets (F-score, \%). $^*$ indicates scores obtained from their released codes. The performance of BERT\_QA\_Arg is lower than that reported in \cite{xinyaduEMNLP2020} as they only consider single-token event triggers. Each score of our approach is the mean of three runs and the variance is shown in parenthesis.
% Argument Ext. (GE) indicates the argument extraction results with gold entities and system predicted triggers. Argument Ext. (GT) indicates the argument extraction performance with gold triggers and system detected entities. 
% *indicate with data augmentation. 
%$^{\star}$ indicates statistical significance $(p < 0.05)$.
%\sijia{$^*$ The result is reproduced by the released code}
}
\label{tab:ACE}
\end{table*}


% % ----------------------------- ERE table ---------------------------
% \begin{table}
% \centering
% \small
% \begin{tabular}{p{3.7cm}|c|c}
% \toprule
% \textbf{Model} & Trigger Ext. & Arg Ext. \\
% \midrule
%     OneIE \cite{yinglinACL2020}             &   57.0  & 46.5  \\
%     BERT\_QA\_Arg \cite{xinyaduEMNLP2020}   &   \multirow{2}{*}{57.0}  &\multirow{2}{*}{39.2}          \\
%     FourIE \cite{vannguyen2021crosstask}    &   57.9  & 48.6  \\
%     Text2Event~\cite{text2event}            & 59.4 & 48.3   \\
% \midrule
%     \textbf{Query\&Extract}                      &   \textbf{60.4}  & \textbf{50.2}  \\
%     % Trained on joint-ontology               &   63.1  & 52.3  \\
% \bottomrule
% \end{tabular}
% \caption{Event extraction F-scores on ERE dataset (\%).}
% \label{tab:ERE}
% \end{table}

% ----------------------------- table ---------------------------
% \begin{table}
% \centering
% \small
% \begin{tabular}{p{2.7cm}|p{1.5cm}<{\centering}|p{1.7cm}<{\centering}}
% \toprule
% Model & Trigger Ext. & Arg Ext. (T) \\ 
% \midrule
% %Zero-Shot~\cite{huang2017zero} & 33.5 & 14.7 \\
% %RCEE~\cite{jianliu2020emnlp} & 5.33 $\dagger$ & ? \\
% BERT\_QA\_Arg \cite{xinyaduEMNLP2020}$^\dagger$ & 31.6 & 17.0 \\
% \midrule
% \textbf{Our Approach} & \textbf{47.8} &  \textbf{43.0}   \\
% % \midrule
% \bottomrule
% \end{tabular}
% \caption{Zero-shot result on 23 unseen event types. $\dagger$ denotes our re-implementation.}
% \label{tab:zeroshot}
% \end{table}
% % ----------------------------- table ---------------------------

% \begin{table*}
% \centering
% \small
% \begin{tabular}{l|c|cc|cc|cc}
% \toprule
% \multirow{2}{*}{Source} & \multirow{2}{*}{Target} & \multicolumn{2}{c|}{BERT\_QA\_Arg$^{1}$} &
% \multicolumn{2}{c|}{BERT\_QA\_Arg$^{2}$} &\multicolumn{2}{c}{\textbf{Our Approach}}  \\ 
% \cmidrule{3-8}
%  &  & Trigger Ext. & Argument Ext. & Trigger Ext. & Argument Ext. & Trigger Ext. & Argument Ext.  \\ 
% \midrule
% ERE & ACE    & 48.9  &  18.5   & 50.8 & 20.9 & 53.9 (52.6)  & 30.2 (29.6) \\
% ACE & ACE    &   &   &   &   & 73.7 &  55.1 \\
% ACE+ERE & ACE & 70.1 & 47.0  & 71.3 & 49.8 & 74.4 (56.3) & 56.2 (41.9) \\ \midrule
% ACE & ERE    &47.2 & 18.0   & 47.2 & 17.9 & 55.9 (46.3) & 31.9 (26.0) \\
% ERE & ERE    &   &    &   &   & 60.4  &  50.2 \\
% ACE+ERE & ERE  &57.0  &  38.6 & 54.6 & 37.1 & 63.1 (51.5) & 52.3 (42.8) \\
% \bottomrule
% \end{tabular}
% \caption{Cross ontology transfer between ACE and ERE datasets. The score in parenthesis indicates the performance on the ACE/ERE shared types on test datasets.}
% %\lifu{In parenthesis, also add the performance on the ACE/ERE shared types on test datasets} \lifu{Reviewers may also ask what happen if we only use annotations for the overlapped types}
% \label{tab:crossontology}
% \end{table*}
% ----------------------------- table ---------------------------

\subsection{Experimental Setup}
%\paragraph{Dataset} 
We perform experiments on two public benchmarks, ACE05-E$^+$\footnote{\url{https://catalog.ldc.upenn.edu/LDC2006T06}} and ERE-EN~\cite{song2015light}\footnote{Following~\citet{yinglinACL2020}, we merge LDC2015E29, LDC2015E68, and LDC2015E78 as the ERE dataset.}.
%Automatic Content Extraction 2005 (ACE05-E$^+$)\footnote{\url{https://catalog.ldc.upenn.edu/LDC2006T06}} and Entity Relation Event (ERE-EN)~\cite{song2015light}\footnote{Following~\citet{yinglinACL2020}, we merge LDC2015E29, LDC2015E68, and LDC2015E78 as the ERE dataset.}. 
ACE defines 33 event types while ERE includes 38 types, among which there are 31 overlapped event types. We use the same data split of ACE and ERE as~\cite{wadden-etal-2019-entity,yinglinACL2020,xinyaduEMNLP2020} for supervised event extraction. For zero-shot event extraction, we use the top-$10$ most popular event types in ACE as seen types for training and treat the remaining 23 event types as unseen for testing, following~\citet{huang2017zero}. In our experiments, we use random seeds
and report averaged scores of each setting. More details regarding the data statistics and evaluation are shown in Appendix~\ref{app:data}.

%Following previous studies~\cite{wadden-etal-2019-entity,xinyaduEMNLP2020,yinglinACL2020}, we ignore \textit{Time} and \textit{Value} related arguments. 

%, including \textit{Facility}, \textit{Geo-Political Entity}, \textit{Location}, \textit{Organization}, \textit{Person}, \textit{Vehicle}, \textit{Weapon}, 

%Appendix~\ref{app:data} shows the detailed statistics of the two datasets. Appendix~\ref{app:imp} provides implementation details. Besides supervised event extraction, we also evaluate our approach with another two settings:

%\paragraph{Supervised Event Extraction} 
%It's a standard supervised learning setting used in most of the previous studies. 
%We conduct experiments for supervised event extraction on ACE and ERE datasets separately. For ACE05-E$^+$, we use the same split as~\cite{qiliACl2013,wadden-etal-2019-entity,yinglinACL2020,xinyaduEMNLP2020}, including 529 documents for training, 30 documents for the development set, and 40 for the test. For ERE-EN, we use the same data split as~\cite{yinglinACL2020, vannguyen2021crosstask}, including 396 documents for training, 31 for the development set, and 31 for the test. %Table \ref{tab:data statistics} shows the details of the data statistics.

%\paragraph{Zero-Shot Event Extraction} To evaluate the transfer capability of our approach, we use the top-$10$ most popular event types in ACE05 as seen types for training\footnote{Including \textit{Attack}, \textit{Transport}, \textit{Die}, \textit{Meet}, \textit{Sentence}, \textit{Arrest-Jail}, \textit{Transfer-Money}, \textit{Elect}, \textit{Transfer-Ownership}, \textit{End-Position}.}, and treat the remaining 23 event types as unseen for testing, following~\citet{huang2017zero}. We use the same data split as supervised event extraction but only keep the event annotations of the 10 seen types for training and development sets and sample 150 sentences with 120 annotated event mentions for the 23 unseen types from the test set for evaluation.

%\paragraph{Cross-ontology Transfer}
We further design two more challenging and practical settings to evaluate how well the approach could leverage resources from different ontologies: (1) \textit{cross-ontology direct transfer}, where we only use the annotations from ACE or ERE for training and directly test the model on another event ontology. This corresponds to the \emph{domain adaptation setting} in transfer learning literature; %This is a more challenging task than the ACE05 zero-shot transfer task described earlier;
(2) \textit{joint-ontology enhancement}, where we take the annotations from both ACE and ERE as the training set and test the approaches on ACE or ERE ontology separately. This corresponds to the \emph{multi-domain learning setting} in transfer learning literature.
Intuitively, an approach with good transferability should benefit more from the enhanced training data from other ontologies. We follow the same train/dev/test splits of ACE and ERE as supervised event extraction.

% \begin{itemize}[leftmargin=*]
% \item \textbf{Supervised Event Extraction}, a standard supervised learning setting used in most of the previous studies. We conduct experiments on ACE and ERE datasets separately. For ACE05, we use the same split as previous work~\cite{qiliACl2013,wadden-etal-2019-entity,yinglinACL2020,xinyaduEMNLP2020}, including 529 documents for training, 30 documents for development set and 40 for test. For ERE, we use the same data split as~\cite{yinglinACL2020, vannguyen2021crosstask}, which includes 396 documents as training set, 31 documents as development set, and 31 documents as test set. Table \ref{tab:data statistics} shows the details of the data statistics.

% \item \textbf{Zero-Shot Event Extraction}, which is to evaluate the transfer learning capability of our approach. Following previous studies~\cite{huang2017zero}, we use the top-$10$ most popular event types in ACE05 as seen types for training, includinng \textit{Attack}, \textit{Transport}, \textit{Die}, \textit{Meet}, \textit{Sentence}, \textit{Arrest-Jail}, \textit{Transfer-Money}, \textit{Elect}, \textit{Transfer-Ownership}, \textit{End-Position}, and treat the remaining 23 event types as unseen types for test. We use the same data split as supervised event extraction, but only keep the event annotations of the 10 seen types for training and development sets, and sample 150 sentences from test set for evaluation, containing 120 annotated event mentions for the 23 unseen types.

% \item \textbf{Cross-ontology Transfer}, a more challenging and practical setting to evaluate how well the approach could benefit from resources and annotations from different ontologies. We explore two different settings: (1) \textit{cross-ontology direct transfer}, where we only use the annotations from ACE or ERE for training, and directly test the model on another target event ontology. This corresponds to the \emph{domain adaptation setting} in transfer learning literature. %This is a more challenging task than the ACE05 zero-shot transfer task described earlier;
% (2) \textit{joint-ontology enhancement}, where we take the annotations from both ACE and ERE as training set, and test the approaches on ACE or ERE ontology separately.
% This corresponds to the \emph{multi-domain learning setting} in transfer learning literature.
% Intuitively, an approach with good transfer capability should benefit more from the enhanced training data from other ontologies.
% \end{itemize}
%i.e., multi-task learning over annotations from multiple ontologies.
%In this setting, we take the annotations from both ACE and ERE as training set, and test the approaches on ACE or ERE target types separately.
% An approach with good transfer capability should benefit more from the enhanced training data from other ontologies.

% \noindent$\bullet$~\textbf{Supervised event extraction}: This is the standard supervised learning setting used in most of the previous studies.
% We conduct experiments on ACE and ERE benchmark datasets separately and compare with published methods. For ACE05, we use the same split as previous work~\cite{qiliACl2013,wadden-etal-2019-entity,yinglinACL2020,xinyaduEMNLP2020}, including 529 documents for training, 30 documents for development set and 40 articles for test. For ERE, we use the same data split as~\cite{yinglinACL2020, vannguyen2021crosstask}, which includes 396 documents as training set, 31 documents as development set, and 31 documents as test set. The details of the data statistics are in Table \ref{tab:data statistics}.

% \noindent$\bullet$\textbf{ACE05 zero-shot extraction}:
% To verify the transfer learning capability of our approach, we further evaluate on a zero-shot event extraction setting following previous studies~\cite{huang2017zero}.
% This setting uses the top-$10$ most popular event types in ACE05 as seen types for training, which includes \textit{Attack}, \textit{Transport}, \textit{Die}, \textit{Meet}, \textit{Sentence}, \textit{Arrest-Jail}, \textit{Transfer-Money}, \textit{Elect}, \textit{Transfer-Ownership}, \textit{End-Position}, and treats the remaining 23 event types as unseen types for testing. 
% For the 10 seen types, we split them to the training and development sets following the same split as the aforementioned supervised task.
% For evaluation, we sample 150 sentences from the test set, including 120 annotated event mentions for the unseen types.

% \noindent$\bullet$\textbf{Cross-ontology transfer}:
% This is a challenging and useful evaluation setting of  transferability.
% We evaluate how well our approach could benefit from resources from different ontologies.
% We design two experimental settings:
% (1) \textbf{cross-ontology zero-shot transfer}, where we only use the annotations from ACE or ERE for training, and directly test the model on another event ontology. This is a more challenging task than the ACE05 zero-shot transfer task described earlier;
% (2) \textbf{joint learning from multiple ontologies}, i.e., multi-task learning over annotations from multiple ontologies.
% In this setting, we take the annotations from both ACE and ERE as training set, and test the approaches on ACE or ERE target types separately.
% An approach with good transfer capability should benefit more from the enhanced training data from other ontologies.


% \paragraph{Implementation Details} 

% For fair comparison with previous baseline approaches, we use the same pre-trained \texttt{bert-large-uncased} model for fine-tuning and optimize our model with BertAdam. We optimize the parameters with grid search: training epoch 10, learning rate $\in [3e\text{-}6, 5e\text{-}5]$, training batch size $\in\{8, 16, 32\}$, dropout rate $\in\{0.4, 0.5, 0.6\}$.
% %\lifu{Add the details of entity detection model}

% \paragraph{Evaluation Criteria} For evaluation, we use the same criteria as~\cite{qiliACl2013,chen2015event,Nguyen2016,yinglinACL2020} as follows:
% \begin{itemize}[leftmargin=*]
%     \item{\textbf{Trigger}: A trigger mention is correct if its span and event type matches a reference trigger.  Each candidate may act as triggers for multiple event occurrences. }
    
%     \item{\textbf{Argument}: An argument prediction is correct only if the event trigger is correctly detected. Meanwhile, its span and argument role need to match a reference argument. An argument candidate  can be involved in multiple events as different roles. Furthermore, within a single event extent, an argument candidate may play multiple roles.}
    
%     % \item{\textbf{Entity}: A Entity mention is correct if its span and entity type matches a reference trigger. }
% \end{itemize}
 


\subsection{Supervised Event Extraction}
\label{sec:sup_event_ext}
%Our first experiment is the standard supervised event extraction on both ACE and ERE.
%Under supervised learning scenario, we leverage annotated data of all the event types.

Table~\ref{tab:ACE} shows the supervised event extraction results of various approaches on ACE and ERE datasets. Though studies~\cite{yang-mitchell-2016-joint,jianliu2020emnlp,xiaoliuACL2018, dbrnn_sha_2018, lai2020emnlp, Veyseh2020EMNLP} have been conducted on the ACE dataset, they follow different settings\footnote{Many studies did not describe their argument extraction setting in detail.}, especially regarding whether the Time and Value arguments are considered and whether all Time-related argument roles are viewed as a single role. Following several recent state-of-the-art studies~\cite{wadden-etal-2019-entity,yinglinACL2020,xinyaduEMNLP2020}, we do not consider Time and Value arguments. Our approach significantly outperforms most of the previous comparable baseline methods, especially on the ERE dataset\footnote{Appendix~\ref{sec:remaining_challenges} describes several remaining challenges identified from the prediction errors on ACE05 dataset.}. Next, we take BERT\_QA\_Arg, a QA\_based method, as the main baseline as it shares similar ideas to our approach to compare their performance. 

%on trigger detection and argument extraction
%The comparison between our approach and the ablated variant without attention mechanisms demonstrates the effectiveness of the attention mechanisms in capturing the correlation between input tokens and event type or argument role queries. 
%To better illustrate the advantage of our approach, we also provide the argument extraction performance based on gold entities or gold triggers as shown in Table~\ref{tab:ACE}. 
%\sijia{Without attention mechanisms, the model will be reduced to the adapted BERT\_QA\_Arg baseline, which shows the impact of our attention mechanisms.} 

% \lifu{emphasize why we don't compare with other baselines}
% \sijia{Previous studies differ in argument detection setting from two aspects, whether the Time and Value arguments are included and whether all Time-related argument roles are viewed as a single role. We follow several state-of-the-art studies and ignore Value and Time arguments. This setting is different from the studies (including ~\cite{jianliu2020emnlp} and ~\cite{xiaoliuACL2018}). \citet{lai2020emnlp} only focuses on trigger detection, while \cite{Veyseh2020EMNLP} only focuses on argument extraction and leveraged external NYT corpus \cite{wang-etal-2019-adversarial-training}. }

%\sijia{Cite , \cite{feng-etal-2016-language}, (?pre for event class > pre for event identification) \cite{cao-etal-2015-improving}, \cite{cleve}}


%\lifu{add the results on MAVEN event detection}\cite{MAVEN}

Specifically, for trigger detection, all the baseline methods treat the event types as symbols and classify each input token into one of the target types or \textit{Other}. So they heavily rely on human annotations and do not perform well when the annotations are not enough. For example, there are only 31 annotated event mentions for \textit{End\_Org} in the ACE05 training dataset, so BERT\_QA\_Arg only achieves 35.3\% F-score. In comparison, our approach leverages the semantic interaction between the input tokens and the event types. Therefore it still performs well when the annotations are limited, e.g., it achieves 66.7\% F-score for \textit{End\_Org}. In addition, by leveraging the rich semantics of event types, our approach also successfully detects event triggers that are rarely seen in the training dataset, e.g., \textit{ousting} and \textit{purge} of \textit{End-Position}, while BERT\_QA\_Arg misses all these triggers. A more detailed discussion about the impact of seed triggers is in Appendix~\ref{sec:impact_seed}.

%on the types of which
%For example, our approach successfully detects \textit{ousting} and \textit{purge} as candidate triggers of \textit{End-Position} while BERT\_QA\_Arg misses all these triggers.

% 14 annotated event annotations for \textit{Extradite} and 31 annotations for \textit{End\_Org} in ACE05 training dataset, so BERT\_QA\_Arg does not perform well, with 66.7\% F-score for \textit{Extradite} and 35.3\% F-score for \textit{End\_Org}. In comparison, our approach mainly relies on the semantic interaction between the input tokens and the event types, therefore it can still perform well even when the annotations are limited, e.g., it achieves 100\% F-score for \textit{Extradite} and 66.7\% F-score for \textit{End\_Org}. In addition, we also notice that by adding prototype event triggers to enrich the semantics of event types, our approach can detect event triggers that are rarely seen in the training dataset. For example, our approach successfully detects \textit{ousting} and \textit{purge} as candidate triggers of \textit{End-Position} events based on its prototype triggers, such as \textit{retired}, \textit{resigned}, while BERT\_QA\_Arg misses all these triggers.

%our approach outperforms BERT\_QA\_Arg on event type \textit{End-Org} by 31.3\% in F1 score, while annotations of type \textit{End-Org} are limited.  \lifu{check the performance of each single event type of our approach and baseline method, and see whether our approach is much better than the baseline method on some types, of which the annotations are not many.}
%\sijia{With additional semantic meaning introduced by prototype trigger, our approach can detect event expressed by rare words. For example, the prototype triggers that we choose for \textit{End-Position} event, "retired" and "resigned",  help detect rare triggers like "ousting" and "purge", which are not detected by BERT\_QA\_Arg. }
%"Beleaguered French media group Vivendi Universal is in advanced negotiations to sell[transfer ownership] its theme park business to a US firm for around 1 . 5 billion dollars , the Los Angeles Times said Friday ."
% Table \ref{tab:ACE} and \ref{tab:ERE} give the experimental results on ACE and ERE, respectively. 
% Our approach outperforms all previous baselines on event detection and argument detection.
%Our approach shows clear advantage on ERE, where it improves over the state-of-the-art by 2.5\% on trigger detection and  1.6\% on argument detection.
%On ACE, we further provide scores of argument extraction with gold entities or gold triggers, in order to decompose the accumulated error from trigger detection and entity detection.

% We see that (1) Our approach outperforms all previous baselines on event detection and argument detection. Especially we achieve 2.5\% improvement on trigger detection and  1.6\% on argument detection on ERE. 
%There are three possible reasons for the improvement in trigger detection: (1) we leverage rich semantics of event types with prototype triggers; (2) we apply attention to capture the semantic correlation between event types and triggers; (3) our approach can deal with overlapped trigger mentions.
% previous work cannot deal with overlapped trigger mentions, therefore, they suffer from inherent systematic error.
% Meanwhile, we emphasize that event mentions can come from a collection of semantic distributions, instead of a single joint distribution\lifu{this sentence is not understandable}. 
% Our approach extends the semantics of event types by leveraging prototype triggers so that the event type representation can capture different semantic variations. 
%\lifu{there could be several reasons that our approach outperforms previous baseline methods: (1) we leverage rich semantics of event types with prototype triggers; (2) we apply attention to capture the semantic correlation between event types and triggers; (3) our approach can deal with overlapped trigger mentions. For each category, provide one example}

% Similarly, for argument extraction, with multiway attention, our approach is able to capture the semantic correlation between the pair of candidate trigger and an entity and each argument role, as well as the underlying semantic connections among all the entities and argument roles, which are proved to provide 

For argument extraction, our approach shows more consistent results than baseline methods. For example, in the sentence ``\textit{Shalom was to fly on to London for talks with British Prime Minister Tony Blair and Foreign Secretary Jack Straw}'', the BERT\_QA\_Arg method correctly predicts \textit{Tony Blair} and \textit{Jack Straw} as \textit{Entity} arguments of the \textit{Meet} event triggered by \textit{talks}, but misses \textit{Shalom}. However, by employing multiway attention, especially the self-attention among all the entities, our approach can capture their underlying semantic relations, e.g., \textit{Shalom} and \textit{Tony Blair} are two persons to talk, so that it successfully predicts all the three \textit{Entity} arguments for the \textit{Meet} event. 

%probably due to the wide context between \textit{Shalom} and \textit{talks}

% able to capture the semantic correlation between the pair of candidate trigger and an entity and each argument role, as well as the underlying semantic connections among all the entities and argument roles, which are proved to provide 

% There could be several reasons that our approach outperforms previous baseline methods in argument detection: (1) The multiway attention enables detection of unapparent arguments. For example, in the sentence "Afterwards Shalom was to fly on to London for talks with British Prime Minister Tony Blair and Foreign Secretary Jack Straw", three entities "Shalom", "Tony Blair" and "Jack Straw" are arguments of the \textit{Meet} event triggered by "talks".  BERT\_QA\_Arg miss one of the entites, "Shalom", possibly due to its far distance to the trigger and the complex verb phrases in between. 
% On the contrary, the person "Shalom" is identified by our approach because it meet both of the taggability requirement (a) has a strong connection with the trigger, and (b) semantically close to the argument role.

%\sijia{(2) The multiway attention can rule out specious arguments. In the following example, "A spokesman said a group of 25 to 30 armed men Wednesday attacked a house ..." BERT\_QA\_Arg mislabeled "house" as \textit{Victim} role of the \textit{Attack} event  triggered by "attacked". On the contrary, the bidirectional attention in our approach enforces the entity align with argument roles. Clearly, a "house" is not a person or group, thus the probability of it being labeled as argument role are diminished.}\lifu{not understandable} 

% \lifu{when you analyze the results, you should compare the test results of approach with one or two baseline methods, and see which events/arguments we predict correctly but the baseline methods did not predict correctly. Use these examples to analyze the reasons}
% ----------------------------- table ---------------------------
% \begin{table}\centering
% \begin{tabular}{lr}
% \toprule
% \textbf{Model} &F1
%  \\
% \midrule
%     JointBeam \cite{qiliACl2013} &67.5 \\
%     JMEE \cite{xiaoliuACL2018} &73.7\\
%     OneIE \cite{yinglinACL2020} &72.8\\
%     BERT\_QA\_Arg \cite{xinyaduEMNLP2020} &72.4\\
%     RCEE \cite{jianliu2020emnlp} &74.9*\\
% \midrule
%     \textbf{Our model} &        73.2\\
%     Trained on joint-ontology&74.4\\
%     ERE &  43.6\\
% \bottomrule
% \end{tabular}
% \caption{Trigger Detection F1 on ACE2005 test set. *indicate with data augmentation.}
% \label{tab:F1table}
% \end{table}
% % ----------------------------- table ---------------------------
% \begin{table}\centering
% \begin{tabular}{lr}
% \toprule
% \textbf{Model} &F1\\
% \midrule
%     OneIE \cite{yinglinACL2020}             &   57.0    \\
%     FourIE \cite{vannguyen2021crosstask}    &   57.9    \\
% \midrule
%     \textbf{Our model}                               &   60.4    \\
%     Trained on joint-ontology               &   \textbf{63.1}    \\
%     ACE               &   55.9    \\
% \bottomrule
% \end{tabular}
% \caption{Trigger Detection F1 on ERE-EN test set}
% \label{tab:F1table}
% \end{table}
% % ----------------------------- table ---------------------------

% ----------------------------- table ---------------------------
% \begin{table}[h]\centering
% \begin{tabular}{lr}
% \toprule
%     {\textbf{Model}} &  F1 \\ 
% \midrule
%     OneIE & 89.6\\
% \midrule
%   BERT+CRF  & 89.3 \\
% \bottomrule
% \end{tabular}
% \caption{Entity Detection}
% \label{tab:F1table}
% \end{table}
% ----------------------------- table ---------------------------

% ----------------------------- table ---------------------------
% \begin{table*}\centering
% \begin{tabular}{lrrr}
% \toprule
% {\textbf{Model}} & Arg Roles &
%  {Known Entity} & Unknown Entity \\ 
% \midrule
%     % JointBeam \cite{qiliACl2013} &- &- \\
%     % JMEE \cite{xiaoliuACL2018} &- &64.7 \\% \cite{jianliu2020emnlp}
%     % OneIE \cite{yinglinACL2020} &-&-\\
%     BERT\_QA\_Arg \cite{xinyaduEMNLP2020} &22& -& 65.36 \\
%     RCEE \cite{jianliu2020emnlp} & 28&  69.0 & - \\
% \midrule
%     \textbf{Our model}       &  22& 71.64 & 67.20\\ 
%     \textbf{Our model}       & 28&72.89  & 66.03\\%70.14\\
% \midrule
%     \textbf{Our model} + ERE (arg21)   & 22   & 72.43 & 68.63\\ 
%     \textbf{Our model} + ERE (arg26)    & 28  & 72.05 ! & 67.26\\
% \midrule
%     ERE (arg21)   & 22   &  &  \\ 
%     ERE (arg26)    & 28  &  \\
% \bottomrule

% \end{tabular}
% \caption{Argument detection F1 given gold trigger. *without data augmentation. }%* drop due to data structure change
% \label{tab:F1table}
% \end{table*}
% ----------------------------- table ---------------------------


% ----------------------------- table ---------------------------
% \begin{table*}[h]\centering
% \begin{tabular}{lrrr}
% \toprule
% {\textbf{Model}} & Arg Roles &
% {Known Entity} & Unknown Entity   \\ 
% \midrule
%     JointBeam \cite{qiliACl2013} & & 52.7&- \\
%     JMEE \cite{xiaoliuACL2018} & &{60.6} &- \\% \cite{jianliu2020emnlp}
%     DYGIE++ \cite{wadden-etal-2019-entity}&22 & -  &51.4\\
%     OneIE \cite{yinglinACL2020} &22&-&54.8\\
%     BERT\_QA\_Arg \cite{xinyaduEMNLP2020}& 22&- & 53.1\\
%     HPNet~\cite{huang_hpn} & 28 & - & 56.8\\
%     RCEE \cite{jianliu2020emnlp} &28& 62.7   &58.7\\

% \midrule
%     \textbf{Our model}    & 22    & 59.68  & 55.09 \\
%     \textbf{Our model}    & 28    & 61.07  & 57.11 \\
% \midrule
%     \textbf{Our model} + ERE (arg21) \textit{(joint training)}  &  22  &  60.51 & 56.21\\ 
%     \textbf{Our model} + ERE (arg26)\textit{ (joint training)}   & 28  &  60.5! & 56.3!\\
% \midrule
%     ERE (arg21) \textit{}  &  22  &   & \\ 
%     ERE (arg26)\textit{}   & 28  & \\
% \bottomrule
% \end{tabular}
% \caption{Argument detection F1 with predicted trigger}
% \label{tab:F1table}
% \end{table*}

% \lifu{Add ERE table and results}

% ----------------------------- table ---------------------------
% \begin{table}\centering
% \begin{tabular}{lrr}
% \toprule
% {\textbf{Model}} &
%  Unk Entity   \\ 
% \midrule
%     OneIE \cite{yinglinACL2020}             &   46.5    \\
%     FourIE \cite{vannguyen2021crosstask}    &   48.6    \\
% \midrule
%     \textbf{Our model} (arg21)   &  50.2  \\ 
%     % Our model (arg26)    &   &  \\
% % \midrule
%     \textbf{Our model} + ACE (arg22)   &  \textbf{52.3}  \\ 
%     ACE    &   \\
% \bottomrule
% \end{tabular}
% \caption{Argument detection F1 with predicted trigger on ERE-EN}
% \label{tab:F1table}
% \end{table}

% % ----------------------------- table ---------------------------
% \begin{table*}[h]\centering
% \begin{tabular}{lrrrr}
% \hline
% \multirow{2}{*}{\textbf{Model}} &
% \multicolumn{2}{c}{\textbf{Known entity}}  &\multicolumn{2}{c}{\textbf{Unknown entity}}    \\ 
% \cmidrule(r){2-3}\cmidrule(lr){4-5}
%  &[Trigger] Known  &Unknown & Known  &Unknown 
%  \\
% \hline
% JointBeam \cite{qiliACl2013} &- & 52.7&-&- \\
% JMEE \cite{xiaoliuACL2018} &- &{60.6}&64.7 ? &- \\% \cite{jianliu2020emnlp}
% OneIE \cite{yinglinACL2020} &-&-&-&56.8\\
% BERT\_QA\_Arg \cite{xinyaduEMNLP2020} & -&-& \textbf{65.36 } & 53.12\\
% RECC \cite{jianliu2020emnlp} &  \textbf{70.1} & 63.6  & 63.6 &59.3\\

% \hline

% \end{tabular}
% \caption{Argument identification F1}
% \label{tab:F1table}
% \end{table*}
% % ----------------------------- table ---------------------------
\begin{table}
\centering
\small
\resizebox{0.45\textwidth}{!}
{
\begin{tabular}{p{2.7cm}|c|c}
\toprule
Model & Trigger Ext. & Arg Ext. (GT) \\ 
\midrule
%Zero-Shot~\cite{huang2017zero} & 33.5 & 14.7 \\
%RCEE~\cite{jianliu2020emnlp} & 5.33 $\dagger$ & ? \\
% BERT\_QA\_Arg \cite{xinyaduEMNLP2020}$^\dagger$ & \multirow{2}{*}{31.6} & \multirow{2}{*}{17.0} \\
BERT\_QA\_Arg$^\dagger$ & 31.6 & 17.0 \\
\midrule
\textbf{Our Approach} & \textbf{47.8} &  \textbf{43.0}   \\
% \midrule
\bottomrule
\end{tabular}
}
\caption{Zero-shot F-scores on 23 unseen event types. $\dagger$: adapted implementation from \cite{xinyaduEMNLP2020}. GT indicates using gold-standard triggers as input.}
\label{tab:zeroshot}
\end{table}

\subsection{Zero-Shot Event Extraction}
\label{subsec:zero-shot}

\begin{table*}[t!]
\centering
\footnotesize
\resizebox{0.95\textwidth}{!}
{
\begin{tabular}{l|c|cc|cc|cc}
\toprule
\multirow{2}{*}{Source} & \multirow{2}{*}{Target} &  \multicolumn{2}{c|}{BERT\_QA\_Arg$_{\textrm{multi}}$}&
\multicolumn{2}{c|}{BERT\_QA\_Arg$_{\textrm{binary}}$$\dagger$} &\multicolumn{2}{c}{\textbf{Our Approach}}  \\ 
\cmidrule{3-8}
 &  & Trigger Ext. & Argument Ext. & Trigger Ext. & Argument Ext. & Trigger Ext. & Argument Ext.  \\ 
\midrule
ERE & ACE    & 48.9 (48.9)  &  18.5 (18.5)   & 50.8 (50.8) & 20.9 (20.9) & 53.9 (52.6)  & 30.2 (29.6) \\
ACE & ACE    & 70.6 & 48.3  & 72.2  & 50.4  & 73.6 &  55.1 \\
% MAVEN & ACE & & -&& -& 12.4 & -\\
% ACE+ERE & ACE & 70.1 & 47.0  & 71.3 & 49.8 & 74.4 (56.3) & 56.2 (41.9) \\ \midrule
ACE+ERE & ACE & 70.1 & 47.0  & 71.3 & 49.8 & 74.4 & 56.2 \\ \midrule
ACE & ERE    &47.2 (47.2) & 18.0 (18.0)  & 47.2 (45.0) & 17.9 (17.1) & 55.9 (46.3) & 31.9 (26.0) \\
ERE & ERE    & 57.0  & 39.2   & 56.7  &  42.9 & 60.4  &  50.4 \\
% ACE+ERE & ERE  &57.0  &  38.6 & 54.6 & 37.1 & 63.1 (51.5) & 52.3 (42.8) \\
ACE+ERE & ERE  &57.0  &  38.6 & 54.6 & 37.1 & 63.0 & 52.3 \\
% \midrule
% ACE & MAVEN     & & - & & - & & -\\
% MAVEN & MAVEN   & & - & & - & 68.8 & - \\
% ACE+MAVEN & MAVEN & & & & & & \\
\bottomrule
\end{tabular}
}
\caption{Cross ontology transfer between ACE and ERE datasets (F-score \%).
%In each block, the first row corresponds to the direct transfer setting and the third corresponds to the enhancement setting.
%We list the in-ontology results (second row) for reference.
The scores in parenthesis indicate the performance on the ACE and ERE shared event types. }
%\lifu{In parenthesis, also add the performance on the ACE/ERE shared types on test datasets} \lifu{Reviewers may also ask what happen if we only use annotations for the overlapped types}
\label{tab:crossontology}
\end{table*}



%As our approach makes great use of the semantics of both event types and argument roles, it's naturally capable of extracting event mentions and arguments for the types that are unseen during training, thus we demonstrate the transfer learning capability of our approach with zero-shot event extraction.

As there are no fully comparable baseline methods for zero-shot event extraction, we adapt one of the most recent states of the arts, BERT\_QA\_Arg~\cite{xinyaduEMNLP2020}, which is expected to have specific transferability due to its QA formulation.
However, the original BERT\_QA\_Arg utilizes a generic query, e.g., ``\textit{trigger}'' or ``\textit{verb}'', to classify each input token into one of the target event types or \textit{Other}, thus is not capable of detecting event mentions for any new event types during the test. We adapt the BERT\_QA\_Arg framework by taking each event type instead of the generic words as a query for event detection. Note that our approach utilizes the event types as queries without prototype triggers for zero-shot event extraction. 
%\sijia{We don't compare with works that use external resources for event representation \cite{zhang-etal-2021-zero} or model pre-training \cite{Lyu-etal-2021-zero}.}

% Our approach makes use of the semantics of both event types and argument roles with a careful design, thus is expected to be capable of extracting events with unseen types during training.
% In this section, we verify this transferability in the zero-shot setting on ACE05.

% As our approach makes great use of the semantics of both event types and argument roles, it's naturally capable of extracting event mentions and arguments for the types that are unseen during training. 
% To evaluate the transfer learning capability, we further design a zero-shot event extraction setting following previous studies~\cite{huang2017zero}, where the top-$10$ most popular event types in ACE05 are used as seen types for training, including \textit{Attack}, \textit{Transport}, \textit{Die}, \textit{Meet}, \textit{Sentence}, \textit{Arrest-Jail}, \textit{Transfer-Money}, \textit{Elect}, \textit{Transfer-Ownership}, \textit{End-Position}, and the remaining 23 event types are taken as unseen types for testing. 
% Specifically, we follow the same data split as Section~\ref{sec:sup_event_ext} and use only the annotations of the 10 event types as the training and development sets. For evaluation, we sample 150 sentences from the test set, including 120 annotated event mentions for the unseen types.
% \begin{figure}
%   \centering
%   \includegraphics[width=.45\textwidth]{zero_shot.png}
%   \caption{Zero-shot event extraction on each unseen event type. The number in parenthesis indicates \# gold event mentions of each unseen type in the test set.}%\sijia{redraw the figure, sort the f1 score in decreasing order}}
%   \vspace{-4mm}
%   \label{fig:zero_shot_error}
% \end{figure}
%To test the ability of mapping contextual information into adequate semantic space, and consequently being able handle new event types, we experiment on zero-shot scenario. Following \cite{huang2017zero}, we train on 10 event types (\textit{Attack}, \textit{Transport}, \textit{Die}, \textit{Meet}, \textit{Sentence}, \textit{Arrest-Jail}, \textit{Transfer-Money}, \textit{Elect}, \textit{Transfer-Ownership}, \textit{End-Position}) and test on the rest 23 (unseen) event types. The training set becomes everything in the original training set except annotations of the 23 unseen event types. For evaluation, we sample 150 sentences from test set, including 120 annotated event mentions of the unseen types. 


% We compare our approach with one of the most recent state-of-the-art BERT\_QA\_Arg~\cite{xinyaduEMNLP2020} framework, which is expected to have certain transferability due to its QA formulation.
% However, the BERT\_QA\_Arg~\cite{xinyaduEMNLP2020} framework still deals with trigger detection as a multi-class classification task.
% That is, it uses a generic query, e.g., ``\textit{trigger}'', to extract event triggers for all the seen training event types, thus is not capable to detect event mentions for any new event types during testing. For fair comparison, we take each event type instead of the generic word ``\textit{trigger}'' as a query for BERT\_QA\_Arg. Note that for zero-shot experiments, our approach also uses only the event types as queries without any prototype triggers. 

% As Table~\ref{tab:zeroshot} shows, our approach significantly outperforms BERT\_QA\_Arg under zero-shot event extraction. The main difference between our approach and BERT\_QA\_Arg lies in the attention mechanism used for trigger and argument extraction. For example, BERT\_QA\_Arg relies on the self-attention within BERT encoder to learn the correlation between event types or argument roles and each input token, while our approach further applies multiple carefully-designed attention mechanisms over BERT contextual representations to better capture the semantic interactions between event types or argument roles and each input token, and among the set of entities or argument roles.

As Table~\ref{tab:zeroshot} shows, our approach significantly outperforms BERT\_QA\_Arg under zero-shot event extraction, with over 16\% F-score gain on trigger detection and 26\% F-score gain on argument extraction. Comparing with BERT\_QA\_Arg, which only relies on the self-attention from the BERT encoder to learn the correlation between the input tokens and the event types or argument roles, our approach further applies multiple carefully designed attention mechanisms over BERT contextual representations to better capture the semantic interaction between event types or argument roles and input tokens, yielding much better accuracy and generalizability. 

% The main difference between our approach and BERT\_QA\_Arg lies in the attention mechanism used for trigger and argument extraction. For example, BERT\_QA\_Arg relies on the self-attention within BERT encoder to learn the correlation between event types or argument roles and each input token, while our approach further applies multiple carefully-designed attention mechanisms over BERT contextual representations to better capture the semantic interactions between event types or argument roles and each input token, and among the set of entities or argument roles.

We further pick 13 unseen event types and analyze our approach's zero-shot event extraction performance on each of them. As shown in Figure~\ref{fig:zero_shot_error}, our approach performs exceptionally well on \textit{Marry}, \textit{Divorce}, \textit{Trial-Hearing}, and \textit{Fine}, but worse on \textit{Sue}, \textit{Release-Parole}, \textit{Charge-Indict}, \textit{Demonstrate}, and \textit{Declare-Bankruptcy}, with two possible reasons: first, the semantics of event types, such as \textit{Marry}, \textit{Divorce}, is more straightforward and explicit than other types, such as \textit{Charge-Indict}, \textit{Declare-Bankruptcy}. Thus our approach can better interpret these types. Second, the diversity of the event triggers for some types, e.g., \textit{Divorce}, is much lower than other types, e.g., \textit{Demonstrate}. For example, among the 9 \textit{Divorce} event triggers, there are only 2 unique strings, i.e., \textit{divorce} and \textit{breakdowns}, while there are 6 unique strings among the 7 event mentions of \textit{Demonstrate}.

\begin{figure}
  \centering
  \includegraphics[width=.45\textwidth]{zero_shot.png}
  \caption{Zero-shot event extraction on each unseen event type. The number in parenthesis indicates \# gold event mentions of each unseen type in the test set.}%\sijia{redraw the figure, sort the f1 score in decreasing order}}
  \label{fig:zero_shot_error}
\end{figure}
%our approach can better capture the semantic interaction between these event type queries and the corresponding candidate triggers. 

%which can be to some extend verified by the diversity of the event triggers for these types. For example, \lifu{XX}. Thus, our approach can better capture the semantic interaction between the candidate triggers and the event types which  %(2) 

% \lifu{semantic diversity of event types} (2) \lifu{transfer of grounding functions between types and tokens}

% Our further analysis reveals the following findings: 
% (1) The performance of trigger detection with BERT\_QA\_ARG heavily depends on BERT, but our approach focuses on the interaction between event query and the context. Though the attention mechanism is embedded in the BERT architecture, our approach further enhances the relationship between the query and context. Therefore, even for unseen event types, our model can derive answers from context. (2) \sijia{not sure in which section to put this point} For argument detection, BERT\_QA\_ARG is unable to distinguish between multiple event triggers within the same sentence. Since the generated question follows the pattern: What/who is the argument\_role in event $X$? Unless the offsets of trigger mentions are specified in the question, it's impossible to distinguish them. \lifu{if the question contains the trigger information, why it cannot distinguish between multiple event triggers?}\sijia{this occurs when the two trigger are the same. For example, in the following sentence, "With a precedant set in Iraq for preemptive \textit{attacks} , Laos will be taken overnight and become a source of invaluable logistics for U . S . military \textit{attacks} on China ." Two "attacks" denotes two event mentions, and the question "Who is the attacking agent in attacks?" cannot distinguish between them.}\lifu{again, add examples to explains these two reasons} \lifu{Also, analyze for both our approach and BERT\_QA\_arg, which types work well and which types don't work} 

%(3) Figure \ref{fig:zero_shot_error} show accuracy in detection unseen event triggers. We see that there are four types performs excellent, which are \textit{Marry}, \textit{Divorce}, \textit{Trial-Hearing} and \textit{Fine}. The first event types have very straight semantic meanings. Through our trigger attention calculation, we can locate the words that aligns with the event type representation. And the event type \textit{Fine} may learn from the seen event type \textit{Transfer-Money}. On the other hand, justice related event types \textit{Sue}, \textit{Release-Parole}, \textit{Convict}, \textit{Charge-Indict} is hard to predict because there is exclusively one justice-related event, \textit{Arrest-Jail}, in the training set. 


%\lifu{(1) analyze why our approach works better than BERT\_QA\_Arg, e.g., show examples, analyze why their approach cannnot capture the semantic correlation between event type query and the tokens } %(2) analyze what types work well, what types don't work, analyze the reasons

%For fair comparison, we adapt the BERT\_QA\_Arg model so that it can handle unseen event types. Specifically, we concatenate event types to the input of trigger detection in BERT\_QA\_Trigger~\cite{xinyaduEMNLP2020}, and adapt the multi-class classifier into a binary classifier, so that it can predict on unseen event types. We also adapt our trigger detection module: since we don't have access to the event mentions of unseen types during training, prototype triggers are not included in event type queries. 
%The experimental result are listed in Table \ref{tab:zeroshot}. 
%\lifu{add descriptions of experimental settings, analyze the results}

%\lifu{provide examples to show the results. Analyze what types work well, and what types don't work well.}

%\lifu{make it clear, for unseen types, we don't use any prototype triggers}




% ----------------------------- table ---------------------------




\subsection{Cross Ontology Transfer}

%\lifu{add cross-ontology transfer results on MAVEN event detection}

% Finally, we evaluate the transfer capability of our approach in the more challenging setting of cross-ontology transfer.
% 
% To illustrate the transfer capability of our approach across different ontologies, we further design two experimental settings: (1) Mutual Enhancement, where we take the annotations from both ACE and ERE as training set, and test the approaches on ACE or ERE target types separately; (2) Directly Transfer, where we only use the annotations from ACE or ERE for training, and directly test the model on another event ontology. 
% 
%We further illustrate the transfer capability of our approach across different ontologies, which is a more challenging and practical setting. 
%Similar as zero-shot event extraction, there is no comparable previous studies f
% For cross-ontology transfer, we develop two variations of BERT\_QA\_Arg as baseline methods: (1) BERT\_QA\_Arg$_{\textrm{multi}}$, which is the same as the original implementation and use multi-classification to detect event triggers. % but trained with only the annotations of overlapped event types from ACE and ERE and evaluated on the whole test set. %. For example, when the source ontology is ERE and the target is ACE, we only use the annotations of the 31 overlapped event types from ERE for training and test the model on the whole test set of ACE. 
% (2) BERT\_QA\_Arg$_{\textrm{binary}}$, for which we apply the same query adaptation as Section~\ref{subsec:zero-shot} and use multiple binary-classification for event detection. % as Section~\ref{subsec:zero-shot}, so it can leverage the whole training dataset from the source ontology
% %To train our approach and BERT\_QA\_Arg$_{\textrm{binary}}$ 
% For \textit{joint-ontology enhancement}, we combine the training datasets of ACE and ERE and optimize the models from scratch.\footnote{Another intuitive training strategy is to sequentially train the model on the source and target ontologies. Our pilot study shows that this strategy performs slightly worse.}

For cross-ontology transfer, we develop two variations of BERT\_QA\_Arg as baseline methods: (1) BERT\_QA\_Arg$_{\textrm{multi}}$, which is the same as the original implementation and use multi-classification to detect event triggers. (2) BERT\_QA\_Arg$_{\textrm{binary}}$, for which we apply the same query adaptation as Section~\ref{subsec:zero-shot} and use multiple binary-classification for event detection. For \textit{joint-ontology enhancement}, we combine the training datasets of ACE and ERE and optimize the models from scratch.\footnote{Another intuitive training strategy is to train the model on the source and target ontologies sequentially. Our pilot study shows that this strategy performs slightly worse.}

% we also explore two strategies: one is to directly train the models on the combination of the annotations from ACE and ERE, and the second strategy is to first pre-train a model on the ontology that is different from the target one, and then fine-tune the model on the annotations of the target ontology. We only report the performance based on the first ontology, which shows better performance in our experiments.\lifu{confirm}\sijia{do yo mean the performance of our approach} 

Table~\ref{tab:crossontology} shows the cross-ontology transfer results in both \emph{direct transfer} and \emph{enhancement} settings. Our approach significantly outperforms the baseline methods under all the settings. Notably, for \emph{direct transfer}, e.g., from ERE to ACE, by comparing the F-scores on the whole test set with the performance on the ACE and ERE shared event types (F-scores shown in parenthesis), our approach not only achieves better performance on the shared event types but also extracts event triggers and arguments for the new event types in ACE. In contrast, the baseline methods hardly extract any events or arguments for the new event types. 
Moreover, by combining the training datasets of ACE and ERE for \textit{joint-ontology enhancement}, our approach's performance can be further boosted compared with using the annotations of the target event ontology only, demonstrating the superior transfer capability across different ontologies. For example, ACE includes a \textit{Transport} event type while ERE defines two more fine-grained types \textit{Transport-Person} and \textit{Transport-Artifact}. By adding the annotations of \textit{Transport-Person} and \textit{Transport-Artifact} from ERE into ACE, our approach can capture the underlying semantic interaction between \textit{Transport}-related event type queries and the corresponding input tokens and thus yield 1.5\% F-score gain on the \textit{Transport} event type of ACE test set. In contrast, both baseline methods fail to be enhanced with additional annotations from a slightly different event ontology without explicitly capturing semantic interaction between event types and input tokens. Appendix~\ref{appendix:cross} provides a more in-depth comparison between our approach and the baseline approaches.
%The only difference between our approach and BERT\_QA\_Arg$_{\textrm{binary}}$ for trigger detection lies in the use of seed triggers in event queries and the
%\lifu{need to add reasons based on the results}

% \sijia{Comparing with MRC-based methods, our approach has two advantages: (1) we use a query that only contains event type-related information and let the model compare the semantics of the input token with the query. In contrast, for QA-based methods, the question consists of noisy information besides the event type like “which is” or “what is.” The model can better find the semantically aligned words with the query than with a question in natural language. That is why our approach performs better than QA-based methods. (2) To improve the semantically matching between the input tokens and the query, we designed several attention mechanisms to capture the contextual correlation of each input token and the query. (3) Many studies \cite{xinyaduEMNLP2020, jianliu2020emnlp} have shown that MRC models are sensitive to the subtle change of the questions, which explains the performance drop of MRC-based methods when tackling event annotations from a different ontology.}


\subsection{Ablation Study}
\label{sec:Ablation}
We further evaluate the impact of each attention mechanism on event trigger detection and argument extraction. As Table~\ref{tab:Ablation} shows, all the attention mechanisms show significant benefit to trigger or argument extraction, especially on the ERE dataset. The Event Type Attention and Multiway Attention show the most effects to trigger and argument extraction, which is understandable as they are designed to capture the correlation between the input texts and the event type or argument role-based queries. We also notice that, without taking entities detected by the BERT-CRF name tagging model as input, but instead considering all the tokens as candidate arguments\footnote{We take consecutive tokens predicted with the same argument role as a single argument span.}, our approach still shows competitive performance for argument extraction compared with the strong baselines. More ablation studies are discussed in Appendix~\ref{sec:more_ablation}.

\begin{table}[h]\centering
\footnotesize
\begin{tabular}{l|l|c|c}
\toprule
& Model & ACE & ERE \\ 
\midrule
\multirow{4}{*}{Trigger} & Our Approach & 73.6 & 60.4\\
& w/o Seed Trigger & 72.2 & 58.2 \\
& w/o In-Context Attention & 72.3 & 57.9\\
& w/o Event Type Attention & 71.1 & 56.9\\
\midrule
\multirow{5}{*}{Arg.} & Our Approach & 55.1 & 50.4\\
%w/o Trigger Info & 51.9 & \\
& w/o Entity Detection & 53.0 & 47.6 \\
& w/o Multiway Attention &  53.4  & 42.8 \\
& w/o Entity Self-attention & 53.7 & 48.3\\
& w/o Arg Role Self-attention & 54.1 & 47.7\\
\bottomrule
\end{tabular}
\caption{Results of various ablation studies. Each score is the average of three runs for each experiment.}
\label{tab:Ablation}
\end{table}

% \begin{table}[h]\centering
% \small
% \begin{tabular}{l|c|c}
% \toprule
% Model & ACE05-E$^+$ & ERE-EN \\ 
% \midrule
% Our Approach & 55.1 & 50.2\\
% %w/o Trigger Info & 51.9 & \\
% w/o Entity Detection & 53.0 & 47.9 \\
% w/o Multiway Attention &  54.0  & 42.2 \\
% w/o Entity Self-attention & & \\
% w/o Arg Role Self-attention & & \\
% \bottomrule
% \end{tabular}
% \caption{Argument Extraction Ablation Study. }
% \label{tab:Ablation}
% \end{table}



% \sijia{Our attention mechanisms aim to capture the correlation between each input token and event type queries or argument roles, while BERT self-attention captures the correlation between each word with all the other contextual tokens. Without enriched contextual representation, the trigger detection module will be reduced to BERT\_QA\_Arg baseline. Without the proposed multi-way attention, the argument detection F1 score drops 1.1\% and 8.0\% on ACE and ERE, respectively. }

% \sijia{Entity information (predicted) is fed into the argument extraction module in the proposed architecture, which indicates argument spans and restricted probable arguments set.  Without that, the argument extraction task reduces to a sequence labeling problem, and F1 drops 2.1\% and 2.3\% on ACE and ERE, respectively.
% }

% ======================= Ablation Table ==============================
% \begin{table}\centering
% \small
% \begin{tabular}{l|c|c}
% \toprule
% Model & ACE05-E$^+$ & ERE \\ 
% \midrule
% Our Approach & 55.1 & 50.2\\
% %w/o Trigger Info & 51.9 & \\
% w/o Entity Info & 53.0 & 47.9 \\
% w/o Multiway Attention &  54.0  & 42.2 \\
% With GT & 68.7 & 67.2\\
% With GT-GE & 74.2 & 72.2\\
% With GE & 59.7 & 59.5 \\
% \bottomrule
% \end{tabular}
% \caption{Argument Extraction Ablation Study. GT: Gold trigger. GE: Gold entities. \sijia{The table will not be included in the final paper, just sit here for now}}
% \label{tab:F1table}
% \end{table}
% ======================= Ablation Table ==============================



% \subsection{Computational and Time Cost}
% Despite the performance improvement via extending from multi-class classification to multiple binary classifications, these approaches usually increase the time cost. We thus design two strategies to mitigate this issue: (1) More than 69\% of the sentences in the training dataset do not contain any event triggers, so we randomly sample 20\% of them for training. 
% %\sijia{(2) We concatenate all the event expressions together with the input sentence, and then retrieve event representations with predefined indices. This gives us an average training time of 2.3h.} (3) 
% (2) Our one-time argument encoding and decoding strategies extract all arguments of each event trigger at once. It is more efficient than the previous QA-based approaches, which only extract arguments for one argument role at once. With these strategies, for trigger detection, our approach takes 80\% more time for training and 19\% less for inference comparing with BERT\_QA\_Arg~\cite{xinyaduEMNLP2020} which relies on multi-class classification for trigger extraction, while for argument extraction, our approach takes 36\% less time for  training and inference than BERT\_QA\_Arg.

\subsection{Pros and Cons of Type-oriented Decoding}
The advantages of our type-oriented binary decoding include: (1) it allows the model to better leverage the semantics of event types which have been proved effective for both supervised and zero-shot event extraction; 
(2) it allows the approach to leverage all available event annotations from distinct ontologies, which is demonstrated in zero-shot event extraction and cross-ontology transfer; (3) in practice, new event types and annotations could emerge incessantly, and it is not possible to always train a model for all the event types. Our approach has the potential to be continuously updated and extract events for any desired event types. 

We also admit that binary decoding usually increases the computation cost. We design two strategies to mitigate this issue: (1) More than 69\% of the sentences in the training dataset do not contain any event triggers, so we randomly sample 20\% of them for training. 
(2) Our one-time argument encoding and decoding strategies extract all arguments of each event trigger at once. It is more efficient than the previous QA-based approaches, which only extract arguments for one argument role at once. With these strategies, for trigger detection, our approach takes 80\% more time for training and 19\% less for inference compared with BERT\_QA\_Arg which relies on multi-class classification, while for argument extraction, our approach takes 36\% less time for training and inference than BERT\_QA\_Arg. Even on a more fine-grained event ontology MAVEN~\cite{MAVEN}, which consists of 168 event types, for trigger extraction, our approach roughly takes 20\% more time for training and twice the time for inference compared with BERT\_QA\_Arg, with slightly better performance than the state of the art~\cite{cleve}\footnote{Our approach achieves 68.8\% F-score on MAVEN. We do not discuss more as MAVEN only contains trigger annotations.}. 

%~\cite{xinyaduEMNLP2020}.
% \sijia{(3)concatenating event types: running time is 2.3h}%  F1: 72.9}

%By extending multi-class classification to multiple binary classification, an evident drawback lies in the high computational and time cost. Fortunately, we designed two strategies to mitigate this issue and ensure our approach to achieve better performance and less time cost for both training and evaluation on the ACE05 dataset than BERT\_QA\_Arg~\cite{xinyaduEMNLP2020} which relies on multi-class classification for trigger extraction: (1) more than 69\% of the sentences in the training dataset do not contain any event triggers, so we randomly sample 20\% of these sentences for training, and (2) our one-time argument encoding and decoding strategies extract all arguments of each event trigger at once. It is more efficient than the previous QA-based approaches, which can only extract arguments for one argument role at once. \sijia{(trainig is 36.3\% faster and inference 36.9\% faster than BERT\_QA\_Arg approach)} \lifu{on which dataset, and do you mean for trigger extraction or trigger and argument extraction?}\sijia{On ACE}
% \sijia{ ACE trigger epoch=10, argument epoch=10, batch_size=16, bert-large
% our approach
% trigger:  avg training >10h,      inference: 7 sentences/s    
            % 102 min with 10%sampling, 157 sentences/s separate bert
% arg       avg training 79 min,    inference: 141 sentence/s}

% BERT_QA_arg
% trigger:  avg training 56 min,    inference: 132  sentences/s
% arg       avg training 124 min,   inference: 103  sentences/s}

% \lifu{add the description in terms of the training and test time cost, compare with OneIE and BERT\_QA\_Arg} \sijia{
% An immediate result of switching from multi-class classification to binary extraction is an increase in computational cost,  however, the increasing amount is limited due to the following reasons  
% (1) More than 69\% of the sentences in the training dataset do not contain any valid event triggers, thus sampling on those training instances can reduce the training time. (2) Our one-time argument encoding and decoding strategies extract all arguments of each event trigger at once. It is more efficient than previous QA-based approaches, which can only extract arguments for one argument role at once. }
%First, our approach excels in the \emph{direct transfer} setting for both transfer directions (ACE $\rightarrow$ ERE and ERE $\rightarrow$ ACE), showing its better transfer capacity compared to the QA-based approaches.
%With the binary classification formulation and our query formulation, we can easily merge new event types into the existing ontology.
%Second, neither of the baselines result in performance boost in the \emph{enhancement} setting, compared to the results without  enhancement (i.e., in-ontology results).
%In comparison, our approach leads to large improvement when trained with the joint of ACE and ERE.

%There are several reasons for our better transferability compared to the previous QA-based approach.\mo{My understanding is that the following bullets are explanations for our improvement in both settings?}
%(1) Our approach enables knowledge transfer between different relevant event types across ontologies. For example, there are two event types "transport: person" and "transport: artifact" in ECE and single "transport" event type in ACE. When trained on ECE, our model learns latent knowledge on transport events of both persons and artifacts. When testing on ACE, this latent knowledge can help us identify transport events of a person or an artifact. The performance for \textit{Transport} type improves by 1.5\% with the new ontology. \lifu{always use numbers and statistics to support your analysis. Here, you should show the test performance on ACE transport event type.}
%In comparison, previous work uses multi-class classification for trigger detection and treats each event type as an independent symbol. 
%(2) The nature of multi-class classification algorithms tends to push event classes far away from each other. Yet in the joint enhancement setting, this does not hold for the "transport", "transport: person" and "transport: artifact".
%Instead, we hope to encourage the knowledge sharing among these related types.
%(3) The cross-entropy loss in multi-class classification also introduces noises.
%For example, when trained on the ACE example with "transport" event, the loss punishes the logits over "transport: person" and "transport: artifact" types.
%Yet the binary classification formulation in our approach avoids such noises. 
% (i) Our approach excels in a cross ontology setting because it can use all annotations from any ontologies. With the binary classification, we can easily merge a new ontology into the existing one. When merging the ontologies, let the queries be the event types/argument roles in the new ontology. And then merge them to the existing ontology, then we are ready for training. 
% (ii) Annotations from other event types can help improve target event types. Previous work that uses the multi-class classification for trigger detection views each event type as an independent annotation. However, under the cross-ontology scenario, there might be closely related annotation types. For example, there are two event types "transport: person" and "transport: artifact" in ECE and single "transport" event type in ACE. When trained on ECE, our model learns latent knowledge on transport person or artifact event. While test on ACE, this latent knowledge can help us identify transport events of a person or an artifact. 
% (iii) Meanwhile, the nature of multi-class classification algorithms tends to push event classes far away from each other. Yet when the source is ACE+ERE, we don't want to push "transport" away from "transport: person" or "transport: artifact". 
% (iv) In our approach, for ACE sentences, we only ask whether any word expresses "transport" event, and for ERE sentences, we only ask whether any word expresses "transport: person" or "transport: artifact" event. Unlike BERT\_QA\_Arg, we'll not introduce errors during data preparation.

% \lifu{For this analysis, we need to emphasize the strentgh of our approach: (1) it can use all annotations from any ontologies; (2) and the annotations from other event types can be helpful for improving target event types} \sijia{shouldn't the second point better fit in analysis for zero-shot scenario?}

%\lifu{which types are enhanced by another ontology based annotations, which are not enhanced. how about the non-overlapped event types?}\sijia{leave the result figure in appendix, seems no space here for it}
%To illustrate the ability of transferring information across different ontologies of our proposed model, we show results under four distinct setting: i) ERE as source ontology and ACE as target ontology, ii) join of ERE and ACE as source and ACE as target, iii) ACE source and ERE target, iv) join of ERE and ACE as source and ERE as target. Settings i) and iii) can reveal model's ability in transferring knowledge to a new ontology, and verify the proper encoding of semantic meanings.

%To compare with BERT\_QA\_Arg, we apply the same adaption as in Section \ref{subsec:zero-shot}. For argument detection of BERT\_QA\_Arg, we manually fill in query questions for each unseen event type in ERE, so that they has associate query questions. 


%\lifu{add experimental results on ACE or ERE with the combined annotations of ACE and ERE, and the evaluation results on ACE with only ERE annotations.}
%\lifu{Use this subsection to show how the approach can leverage annotations from different ontologies}

% \lifu{We may need to split the performance on the ACE/ERE shared types and distinct types. Reviewers may ask whether the 43.6 Fscore is just from the shared event types}\sijia{It turns out to be a mistake in my code, it should be 53.89}




%During our experiment, we find the word "talks" being particularly difficult to predict. There are 28 occurrences of "talks" in the ACE test set, and 10 of them are annotated as \textit{Contact-Meet} events. However, when we evaluate on the test set, our model tends to label most of them as "contact-meet" events. By the annotation rule in ACE~\cite{ldc_ace05}, we know that this event has very restricted taggability rules. For example, it requires two or more parties to physically get together at some location. Though our in-context attention is meant to capture the relationship between the candidate trigger and the context, in this case, the result indicates stronger relation measure is needed. 


==> ACL 2022_ Refining Event Extraction as Type-oriented Binary Decoding/4related_work.tex <==
\section{Related Work}
\label{sec:related}
% should be argument detection instead of argument classification 
% ACE has overlap arguments 
% ERE has overlap triggers and arguments 
% The evaluation is spurious
%
% In this section, we briefly describe prior work from the areas of event extraction and heterogeneous graph embedding that are most related to our work.

% Since single candidate span may act as triggers for multiple event occurrences, traditional frameworks that separates trigger identification and classification suffer from systematic error. 

%Event extraction has been a long-studied and challenging task in natural language processing (NLP)~\cite{Riloff1996, qiliACl2013, wadden-etal-2019-entity}. 

% , based on hand-crafted features or deep embedding based features~\cite{pennington2014glove,peters2018deep,devlin-etal-2019-bert}

Traditional event extraction studies~\cite{mcclosky2011event,qiliACl2013,chen2015event,cao-etal-2015-improving,feng-etal-2016-language,yang-mitchell-2016-joint,nguyen_jrnn_2016,zhang2017improving,wadden-etal-2019-entity,yinglinACL2020,cleve} usually detect event triggers and arguments with multi-class classifiers. Unlike all these methods that treat event types and argument roles as symbols, our approach considers them queries with rich semantics and leverages the semantic interaction between input tokens and each event type or argument role.

Several studies have explored the semantics of event types based on seed event triggers~\cite{bronstein2015seed,lai2019extending,zhang-etal-2021-zero}, event type structures~\cite{huang2016liberal,huang2017zero}, definitions~\cite{chen2019reading} and latent representations~\cite{huang2020semi}. However, they can hardly be generalized to argument extraction. Question answering based event extraction~\cite{xinyaduEMNLP2020, jianliu2020emnlp, EEMQA_li, Lyu-etal-2021-zero} can take advantage of the semantics of event types and the large-scale question answering datasets. Compared with these methods, there are three different vital designs, making our approach perform and be generalized better than these QA-based approaches: (1) our approach directly takes event types and argument roles as queries. In contrast, previous QA-based approaches rely on templates or generative modules to create natural language questions. However, it is difficult to find the optimal format of questions for each event type, and many studies \cite{xinyaduEMNLP2020, li-etal-2020-unified} have shown that MRC or QA models are sensitive to the subtle change of the questions.
(2) QA-based approaches can only detect arguments for one argument role at once, while our approach extracts all arguments of an event trigger with one-time encoding and decoding, which is more efficient and leverages the implicit relations among the candidate arguments or argument roles. (3) QA-based approaches rely on span prediction to extract arguments without requiring entity extraction, which could result in more entity boundary errors. Thus we choose to pre-train a name tagging model and use binary decoding over system detected entities.Moreover, it is pretty challenging to fully adapt the event extraction task to the span-based Question Answering. The main reason is that each sentence may contain multiple triggers for a particular event type. Even if we can formalize a question, e.g., “what is the trigger for Attack?” it is difficult for the model to return all the spans of event triggers correctly.

% (1) we use a query which only contains event type related information, e.g., event type name or seed triggers, and expect the model to compare the semantic consistency of each input token with the query and determine if the token should be a mention of the query or not, while for MRC-based methods, the question usually consists of other noisy information besides the event type, e.g., “what’s the event trigger of attack?”. It’s easier for the model to find the words that are semantically aligned with the query than interpreting the meaning of the question and then finding the answer from the input sentence, and that’s why our approach performs better than MRC-based methods; (2) to improve the semantically matching between the input tokens and the query, we designed several attention mechanisms to capture the meaningful contextual information of each input token as well as the contextual representation of query. (3) a lot of studies [1, 2] have shown that MRC models are sensitive to the subtle change of the questions, which could be another potential reason that by introducing event annotations from a different ontology, the performance of MRC-based methods drops a little.


% \sijia{should we compare with other prompt-based approaches? 
% 1) TANL \cite{tanl}: % https://arxiv.org/abs/2101.05779
% 2) TEXT2EVENT \cite{text2event} % https://arxiv.org/pdf/2106.09232.pdf
% }
%Comparing with these methods, our approach further models event extraction with binary decoding by leveraging the semantic interaction between input text and the event type queries, yielding much higher accuracy and stronger capability for zero-shot and cross-ontology transfer. 
%In addition, for each event mention, our framework efficiently extracts all candidate arguments with one-time encoding without creating any questions repeatedly, thus is more computationally efficient. 

%propose to model event extraction as a question answering task and extract triggers and arguments by finding the answers to the questions that are defined by templates or automatically generated. Our approach share similar ideas as these work but ...

%their definitions, event type structures and example event mentions, with the goal of improving the transferability and portability of the event extraction approaches. For example, XX utilize an event type structures to characterize the semantic meanings of each event type and ground each candidate event mention or argument to a corresponding type or argument role based on their similarity.~\newcite{} leverage event type definitions to .... Additionally, ~\newcite{} introduce several example event mentions to learn the .. Comparing with these studies, our approach not only consider the semantics of each event type and argument role, but also fully captures the interaction between the local context and the type or argument role, which was rarely explored by previous studies.

% Finally, several recent work~\cite{xinyaduEMNLP2020, jianliu2020emnlp, EEMQA_li},  propose to model event extraction as a question answering task and extract triggers and arguments by finding the answers to the questions that are defined by templates or automatically generated. Our approach share similar ideas as these work but ...

% EE is a crucial IE task that aims to extract event information in texts, which has attracted extensive attention among researchers. Traditional EE methods employ manual-designed features, such as the syntactic feature (Ahn, 2006), document-level feature

% \lifu{semantic enriched event extraction, e.g., QA based, structure/example/definition based}

    

==> ACL 2022_ Refining Event Extraction as Type-oriented Binary Decoding/5conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}
% In this paper, we presented a novel graph neural network based framework - $\emph{SemPathNet}$ - an end-to-end modeling framework for heterogeneous graph embedding. Our experiments are conducted on two scenarios, i.e., node classification and node clustering. The experimental results illustrate that $\emph{SemPathNet}$ outperforms various state-of-the-art models.

We refine event extraction with a query-and-extract paradigm and design a new framework that leverages rich semantics of event types and argument roles and captures their interactions with input texts using attention mechanisms to extract event triggers and arguments. Experimental results demonstrate that our approach achieves state-of-the-art performance on supervised event extraction and shows prominent accuracy and generalizability to new event types and across ontologies. In the future, we will explore better representations of event types and argument roles and combine them prompt tuning approach further to improve the accuracy and generalizability of event extraction.


%\sijia{ We plan to summarize previous different settings for a fair comparison.
%From various efforts on Event Extraction tasks, we found that a standard evaluation method is missing. Previous work varies in dataset pre-processing and task formulations, such as the argument types considered. We also plan to investigate the effect of different query strategies. The proposed event representation is representative but sub-optimal. Seed triggers are semantically meaningful and can align nicely with high-frequency trigger candidates. However, they could boost the possibility of making a false positive prediction on related tokens and omitting unseen or rare candidates.}

%extend our framework to other information extraction tasks and to leverage available annotations from related tasks.

%Experiments on supervised event extraction, zero-shot event extraction as well as cross-ontology transfer with two public benchmark datasets ACE and ERE demonstrate that our approach not only yields more accurate 


